FedBC: Calibrating Global and Local Models via Federated Learning Beyond Consensus

In this work, we quantitatively calibrate the performance of global and local models in federated learning through a multi-criterion optimization-based framework, which we cast as a constrained program. The objective of a device is its local objective, which it seeks to minimize while satisfying nonlinear constraints that quantify the proximity between the local and the global model. By considering the Lagrangian relaxation of this problem, we develop a novel primal-dual method called Federated Learning Beyond Consensus (\texttt{FedBC}). Theoretically, we establish that \texttt{FedBC} converges to a first-order stationary point at rates that matches the state of the art, up to an additional error term that depends on a tolerance parameter introduced to scalarize the multi-criterion formulation. Finally, we demonstrate that \texttt{FedBC} balances the global and local model test accuracy metrics across a suite of datasets (Synthetic, MNIST, CIFAR-10, Shakespeare), achieving competitive performance with state-of-the-art.

==> sections/Simulations.tex <==
%!TEX root = main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% S  E  C  T  I  O  N%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% F   I   G   U   R   E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\section{Simulations} \label{sec:simulations}
%\begin{figure}[t]
%	%\centering
%	\vspace{4mm}
%	\centerline{\includegraphics[width=.9\columnwidth,clip = true]{figs/l17.png}}
%	\vspace{0mm}   
%	%\centerline{\hspace*{0.6cm}\footnotesize(a)\hspace*{4.3cm}(b)}
%	{{\centering  
%	\caption{Environment with misleading rewards} \label{fig:env}}}\vspace{-4mm} 
%\end{figure} 
In this section, we  first  validate the  efficacy of  proposed policy parameterizations using the  custom-made environment  of Section \ref{sec:prob}.   Further, we implement  the  considered parameterizations in the standard continuous mountain car environment  of  OpenAI gym. 
\subsection{Custom-made Environment:  Car Trapped Between two Mountains}
At each episode, the car is always initialized within a small neighborhood $[1.15,2.0]$.   
States, $x$ is constrained  to an interval  $[-4.0, \,  3.709]$ and $a_t$ lies in $[-20, \, 20]$. The discounted factor $\gamma$ is  $0.97$  and we use   a diminishing step-size ranging from 0.005 to $5 \times 10^{-9}$.
Next we present performance comparison of the policy parameterizations, Examples \ref{eg:gaussian_fixed_var}- \ref{eg:alpha_stable} for the custom-made environment. 
% -- this parameterization satisfies Assumption \ref{assum:regularity_for_CNC}. 
\subsubsection{$S \alpha S$   distributions  with constant scale}
We evaluate the performance of $S \alpha S$ stable distributions  with constant scale for $\alpha$ values of one and two. In other words, this corresponds to Gaussian and Cauchy policy of  \eqref{eq:Gaussian_policy} and \eqref{eq:Cauchy_policy} with a constant $\sigma$. 
%Cauchy policy for constant sigma is given by 
%\begin{align}
%\pi_{\bm{\theta}}(a|s) = \frac{1}{\sigma \pi (1+(\frac{a-x_0}{\sigma})^2) }
%\end{align}
% Corresponding score function with constant sigma (only $x_0$ is parameterized as $x_0 = \bm{\theta}^\top_{x_0}s$, $\bm{\theta}=[\bm{\theta}_{x_0}]$) is given by 
%\begin{align}
%\nabla_{\bm{\theta}} \log \pi_{\bm{\theta}} (s,a) = \left[
%\begin{matrix}
% \frac{2}{1+ \left( \frac{(a-\bm{\theta}_{x_0}^\top s)}{\sigma}\right)^2} \left(  \frac{a-\bm{\theta}_{x_0}^\top s}{\sigma^2} \right)  s
%\end{matrix}
%\right]
%\end{align}
%Gaussian Policy with constant variance takes the following  form
%\begin{align*}
%\pi_{\bm{\theta}}(a|s) = \mathcal{N} (a|s^\top \bm{\theta}, \sigma^2)
%\end{align*}
%Corresponding score function with constant sigma,  $\bm{\theta}=[\bm{\theta}_{\mu}]$
%\begin{align}
%\nabla_{\bm{\theta} }  \log \pi_{\bm{\theta}} (s,a)= (a-s^\top \bm{\theta}_{\mu})s/\sigma^2
%\end{align}
Numerical experiments here consider a fixed scale of  1.0. Figure \,\ref{fig:1} shows the cumulative  return averaged over   latest 100 episodes.  Heavy tailed Cauchy distribution drives the car to the desired goal post and converges faster than standard Gaussian. However,  as evident from the figure, both policies exhibit high variance.  Though heavy-tailed distribution achieves better performance,  policy leads to the misleading goal at certain instants. The result hints at the necessity of variable scale of $S \alpha S $  distributions.
\begin{figure}[t]
	%\centering
	\vspace{4mm}
	\centerline{\includegraphics[width=.9\columnwidth,clip = true]{figs/Figure_2tru_var.png}}
	\vspace{0mm}   
	%\centerline{\hspace*{0.6cm}\footnotesize(a)\hspace*{4.3cm}(b)}
	{{\centering  
	\caption{Custom made environment with misleading rewards: Average cumulative returns  over latest 100 episodes for  policies with constant sigma. Cauchy policy reaches desired goal post and Gaussian settles to sup-optima. } \label{fig:1}}}\vspace{-4mm} 
\end{figure} 
% \begin{figure}[t]
%	%\centering
%	\vspace{4mm}
%	\centerline{\includegraphics[width=.9\columnwidth,clip = true]{figs/Figure_1gctru_var.png}}
%	\vspace{0mm}   
%	%\centerline{\hspace*{0.6cm}\footnotesize(a)\hspace*{4.3cm}(b)}
%	{{\centering  
%	\caption{Constant sigma:   cumulative discounted returns } \label{fig:2}}}\vspace{-4mm} 
%\end{figure} 
\subsubsection{$S \alpha S$  stable distributions  with variable scale}
This section considers the performance of variable scale policy parameterization of Example  \ref{eg:alpha_stable} in the custom-made environment.
% of Cauchy and variance of Gaussian policies are also parameterized as $\sigma = \exp^{\bm{\theta}_{\sigma}}$ $\bm{\theta}=[\bm{\theta}_{x_0}, \bm{\theta}_{\sigma}]$. The corresponding score function for Cauchy and Gaussian policies are given by 
%\begin{align}
%&\nabla_{\bm{\theta} } \log \pi_{\bm{\theta}} (s,a) = \left[
%\begin{matrix}
% \frac{2}{1+ \left( \frac{(a-\bm{\theta}_{x_0}^\top s)}{\sigma}\right)^2} \left(  \frac{a-\bm{\theta}_{x_0}^\top s}{\sigma^2} \right)  s
% \\ -\bold{1} + \frac{2}{1+ \left( \frac{a-\bm{\theta}_{x_0}^\top s}{\sigma}\right)^2} \left(a-\bm{\theta}_{x_0}^\top s\right)^2 \sigma^{-2} 
%\end{matrix}
%\right]
%\\
%& \nabla_{\bm{\theta} } \log \pi_{\bm{\theta}} (s,a)= 
%\begin{bmatrix}
%\frac{(a-s^\top\bm{\theta}_{\mu})s}{\sigma^2}  \\
%\frac{\left(a-s^\top \bm{\theta}_{\mu}\right)^2}{\sigma^2}-1
%\end{bmatrix}
%\end{align} 
The unbounded score function and related divergence issues in the implementation are taken care of using projected policy gradients of Algorithm \ref{Algorithm1}.
   Figure \ref{fig:3} shows the average cumulative returns for both the policies.  Both Cauchy and Gaussian policy reach to desired goal post with better convergence for increased tail index.   Besides, the Cauchy policy exhibits less variance. Results hint at the predominant persistent exploration property with a decrease in the tail index discussed in Section \ref{sec:prob}.
 \begin{figure}[t]
	%\centering
	\vspace{4mm}
	\centerline{\includegraphics[width=.9\columnwidth,clip = true]{figs/Figure_2_sg2.png}}
	\vspace{0mm}   
	%\centerline{\hspace*{0.6cm}\footnotesize(a)\hspace*{4.3cm}(b)}
	{{\centering  
	\caption{Custom made environment with misleading rewards: Average cumulative returns  over latest 100 episodes for  policies with variable sigma. Cauchy policy shows faster convergence.}
	\label{fig:3}}}\vspace{-4mm} 
\end{figure} 
% \begin{figure}[t]
%	%\centering
%	\vspace{4mm}
%	\centerline{\includegraphics[width=.9\columnwidth,clip = true]{figs/Figure_1_sg2.png}}
%	\vspace{0mm}   
%	%\centerline{\hspace*{0.6cm}\footnotesize(a)\hspace*{4.3cm}(b)}
%	{{\centering  
%	\caption{Variable  sigma: cumulative discounted returns } \label{fig:4}}}\vspace{-4mm} 
%\end{figure} 
Now, we consider an interesting scenario where each episode starts from the false goal point.  In comparison with the previous case, both policies take more time to escape the false goal post.  However, results indicate    the relatively less first-exit time of the heavy tailed distribution as shown in Fig \ref{fig:5}
 \begin{figure}[t]
	\centerline{\includegraphics[width=.9\columnwidth,clip = true]{figs/Figure_2_sg2_trp.png}}
	\vspace{0mm}   
	%\centerline{\hspace*{0.6cm}\footnotesize(a)\hspace*{4.3cm}(b)}
	{{\centering  
		\caption{Custom made environment with misleading rewards: Average cumulative returns  over latest 100 episodes for  policies with variable sigma where each episode is initialized at the local basin of attraction.  Cauchy policy takes less time to exit spurious local minima as compared to Gaussian policy.}
 \label{fig:5}}}
\end{figure} 
% \begin{figure}[t]
%	%\centering
%	\centerline{\includegraphics[width=.9\columnwidth,clip = true]{figs/Figure_1_sg2_trp.png}}
%	\vspace{0mm}   
%	%\centerline{\hspace*{0.6cm}\footnotesize(a)\hspace*{4.3cm}(b)}
%	{{\centering  
%	\caption{Initial conditions in local basin of attraction:  cumulative discounted  returns during episodes  } \label{fig:6}}}
%\end{figure} 
%Recall that the length of the rollout horizon for Q-function  estimate in our algorithm is drawn from $\text{Geom}(1-\gamma^{1/2})$.} 
%After each rollout, i.e., one episode, the policy parameter $\theta_k$ is updated and then evaluated by calculating the value of $J(\theta)$ using the Monte-Carlo method. 
%Recall that Algorithm \ref{alg:RPG} is termed as RPG. 
%Moreover,  we refer to Algorithm \ref{alg:MRPG} that uses intermittently larger stepsizes with stochastic policy gradient $\hat{\nabla}J(\theta)$ as \emph{MRPG$_1$}. 
%
%In order to verify  the significance of  the CNC condition  in escaping saddle points, we also test the MRPG$_1$ algorithm in the environment that has mixed reward, i.e., the reward can be both positive and negative. We generate such an environment by  adding a constant $10.0$ onto the reward defined in  \eqref{equ:reward_Pendulum}. Each learning curve in Figure \ref{fig:offset_comp} is run for $30$ times, and the bar area in the figure represents plus or minus one sample standard deviation of $30$ trajectories. %
%

\subsection{Continuous Mountain car in OpenAI gym}
In this section we evaluate the performance of policy parameterization on continuous mountain car from OpenAI gym environment. Parameters of the Algorithm are identical to the previous case.  Environment represents a a one-dimensional track of a car positioned between two mountains.  The goal is to drive up the mountain on the right; of course and the only way to succeed is to drive back and forth to build up momentum. The observation of mountain car is given by its  horizontal position x and  velocity v. In this experiment, the reward of $-1$ is given for every time step when the car remains between two mountains and  the episode ends when the car reaches desired target height. Figure \ref{fig:6} shows  cumulative average return for  variable scale $S \alpha S$ distributions  of  Example \ref{eg:alpha_stable} with $\alpha = 1,\, 2 $.  Heavy-tailed distribution better explore the space and settles to the optimal action. Average cumulative return using Gaussian policy shows sluggish performance. Results again validate  the effectiveness of heavy tailed distributions in better exploring the action space.  
\begin{figure}[t]
	\centering
	\vspace{4mm}
	\centerline{\includegraphics[width=.9\columnwidth,clip = true]{figs/Fig_mc1.png}}
	\vspace{0mm}   
	\centerline{\hspace*{0.6cm}\footnotesize(a)\hspace*{4.3cm}(b)}
	{{\centering  
	\caption{Continuous Mountain car in OpenAI gym: Average cumulative returns  over latest 100 episodes for  $S \alpha S$ policies with variable scale. Heavy tailed policy (Cauchy) reaches desired goal post and Gaussian shows sluggish response. } \label{fig:6}}}\vspace{-4mm} 
\end{figure} 

==> sections/convergence_amrit.tex <==
%!TEX root = main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Following discussion establishes the convergence of these exploratory policies to first-order stationary points. First we establish convergence of the proposed policy class  without adaptive variance and then we extend it to  exploratory search with adaptive variance.  
\section{Convergence Analysis} \label{sec:convergence}
First we state the assumptions and notions used in the paper. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Assumptions}
\begin{assumption} \label{Assum:Q}
The reward function, $R$ and the parameterized policy, $\pi_{\bm{\theta}}$ satisfies the 
following properties:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{enumerate}
\item The absolute value of the reward is uniformly bounded,
$$
\sup_{(s,a) \in \mathcal{S} \times \mathcal{A}} |R(s,a)|  \leq  U_R, U_R < \infty.
$$
\item For all $ \, \bm{\bm{\theta}}_1, \, \bm{\theta}_2 \in \mathbb{R}^p$, the continuous policy, $\pi_{\bm{\theta}}$  is such that
 $\pi_{\bm{\theta}} \in \mathcal{C}^{1,1}$
\begin{align}
& | \pi_{\bm{\bm{\theta}}_1}(\cdot|s)  - \pi_{\bm{\bm{\theta}}_2}(\cdot|s )| \leq L_0(\pi) \|\bm{\bm{\theta}}_1-\bm{\bm{\theta}}_2\|, \label{eqn:c0}
\\
& \| \nabla \pi_{\bm{\bm{\theta}}_1}(\cdot|s)  - \nabla \pi_{\bm{\bm{\theta}}_2}(\cdot|s ) \| \leq L_1 (\pi) \|\bm{\bm{\theta}}_1-\bm{\bm{\theta}}_2\|.    \label{eqn:c1}
\end{align}
\end{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The direct consequence of condition 1 is a bounded Q-function given by $U_{R}/(1-\gamma)$ which implies  bounded norm on $J(\bm{\theta})$  as well.
\end{assumption}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 We define  $L_{\pi}(\bm{\theta},s) \in \mathcal{C}^{1,1}$
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align} \label{Eqn:bL}
|L_{\pi}(\bm{\theta}_1,s)-L_{\pi}(\bm{\theta}_2,s)| \leq L_0(L_{\pi}) \|\bm{\theta}_1 -\bm{\theta}_2\|.
\end{align}
\begin{align} \label{Eqn:bL1}
\|\nabla L_{\pi}(\bm{\theta}_1,s)-\nabla L_{\pi}(\bm{\theta}_2,s) \| \leq L_1(L_{\pi}) \|\bm{\theta}_1 -\bm{\theta}_2\|.
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 Now the  policy gradient can be expressed as 
\begin{align} \label{Eqn:grad_j1}
&{\nabla} _{\bm{\theta}} J_{\mu}(\bm{\theta})  = \frac{1}{(1-\gamma)} \sum_{s} (1-\gamma)  \rho_{\pi_{\bm{\theta}}}(s) \nonumber \\ 
&  \mathbb{E}_{a \sim \pi_{\bm{\theta}}(\cdot|s)} \left[ \hat{Q}_{\pi_{\bm{\theta}}}(s,a)  \nabla_{\bm{\theta}} \log \pi_{\bm{\theta}}(a|s) \right].  
\end{align} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 The update of the policy parameters is similar to stochastic gradient ascent and we can adopt  non-convex stochastic setting to analyze convergence  to first-order stationary point. 
%
\begin{definition}{(First-order stationary points)}  \label{def:1}
For a twice differentiable objective function  ${J} : \mathbb{R}^d \to  \mathbb{R}$, we say that $\bm{\theta}$ is an $\epsilon$ first order stationary point (FOSP) if 
\begin{align}
\|\nabla J(\bm{\theta}) \|  < \epsilon.
\end{align} 
\end{definition}
Next, we look into the convergence guarantees of the above approach to first-order stationary point.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{assumption}
The estimate of stochastic gradient satisfies the following assumption,
\begin{align}
\mathbb{E} \left[ \| \hat{\nabla} J(\bm{\theta}) \|^2  \right] \leq m +n \|\nabla J( \bm{\theta}) \|^2
\end{align}
\end{assumption}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Let us start the analysis by re-writing  the gradient updated  as %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}\label{udpate11}
\bm{\theta}_{k+1} =  & \bm{\theta}_k  +\alpha_k { \nabla} J(\bm{\theta}_k)
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 We note that the update for $\bm{\theta}_k$ in \eqref{udpate11} can be equivalently written as 
%
\begin{align}\label{optimization_problem}
\bm{\theta}_{k+1} = \argmax_{\bm{\theta} } J(\bm{\theta}_{k} )+\langle{ \nabla} J(\bm{\theta}_k),\bm{\theta}-\bm{\theta}_k\rangle-\frac{1}{2\alpha_k}\|\bm{\theta}-\bm{\theta}_k\|^2.
\end{align}
%
 We can obtain the update in \eqref{udpate11} from the optimality of unconstrained optimization in \eqref{optimization_problem}. In a more general setting, the last term $\|\bm{\theta}-\bm{\theta}_k\|^2$ could be replaced by the Bregman divergence term. The first two terms in the objective of \eqref{optimization_problem} is nothing but the first order approximation of the non-convex objective $J(\bm\theta)$ at $\bm\theta_k$. In order to incorporate the local geometrical structure [\textcolor{red}{might require some more motivation}], we proposed to use the quadratic lower bound provided by the Lipchitz property of the objective, which implies that

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}\label{new_approximation}
 J (\bm{\bm{\theta}}) \geq &  J (\bm{\bm{\theta}}_{k}) +  \left<{\nabla} J (\bm{\bm{\theta}}_k), \bm{\theta}_{k+1} -\bm{\theta}_{k} \right> 
 \nonumber
 \\
 &- 
   \frac{L_1(J)}{2}  \left\|  \bm{\theta}-  \bm{\theta}_{k}    \right\|^2. 
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Now using the second order lower bound \eqref{new_approximation} into \eqref{optimization_problem}, we can write the update
%
\begin{align}\label{optimization_problem22}
	\bm{\theta}_{k+1} = \argmax_{\bm{\theta} } & \ J(\bm{\theta}_{k} )+\langle{ \nabla} J(\bm{\theta}_k),\bm{\theta}-\bm{\theta}_k\rangle\nonumber
	\\
	&\quad-\left(\frac{1}{2\alpha_k}+\frac{L_1(J)}{2}\right)\|\bm{\theta}-\bm{\theta}_k\|^2.
\end{align}
%
The updated problem implies the following update 
%
\begin{align}\label{update2}
	\bm{\theta}_{k+1} =  & \bm{\theta}_k  +\left(\frac{1}{\alpha_k}-{L_1(J)}\right)^{-1} { \nabla} J(\bm{\theta}_k).
\end{align}
%
The stochastic version of the update is given by 
%
\begin{align}\label{stochastic}
	\bm{\theta}_{k+1} =  & \bm{\theta}_k  +\left(\frac{1}{\alpha_k}-{L_1(J)}\right)^{-1} { \hat\nabla} J(\bm{\theta}_k).
\end{align}
%
where ${ \hat\nabla} J(\bm{\theta}_k)={\nabla} J(\bm{\theta}_k)+\bm w_k$ is the stochastic estimate of the true gradient with error $\bm w_k$. The error sequence is assumed to have the following properties
%
\begin{assumption}
	The error sequence 
	
	i) is zero mean $\mathbb{E} \left[ \bm{w}_k |\mathcal{F}_k   \right] =  0$, 
	
	ii) and have bounded second moment as 
	\begin{align}
		\mathbb{E} \left[ \|\bm{w}_k\|^2 |\mathcal{F}_k   \right] = & Y_1 +Y_2 \|\nabla J(\bm{\theta}_k)\|^2 \, 
	\end{align}
for some constant $Y_1, Y_2>0$.
\end{assumption}

\begin{theorem}[Sample complexity]

\end{theorem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
& J (\bm{\bm{\theta}}_{k}) +  \left<{\nabla} J (\bm{\bm{\theta}}_k), \bm{\theta}_{k+1} -\bm{\theta}_{k} \right> - 
   \frac{1}{2} \alpha_k^2 L_1(J) \left\|  \bm{\theta}_{k+1} -  \bm{\theta}_{k}    \right\|^2 \geq  \nonumber \\ &  J (\bm{\bm{\theta}}_{k}) + \alpha_k \left<{\nabla} J (\bm{\bm{\theta}}_k), \nabla J(\bm{\theta}_k)- \bm{w}_k  \right> +
 \nonumber \\ &  \frac{1}{2} \alpha_k^2 L_1(J) \left\|  \nabla J(\bm{\theta}_k)-\bm{w}_k    \right\|^2. 
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Using triangular  inequality for norms, the above expression simplifies to 
 \begin{align}
&  J (\bm{\bm{\theta}}_{k}) + \alpha_k \left<{\nabla} J (\bm{\bm{\theta}}_k), \nabla J(\bm{\theta}_k)- \bm{w}_k   \right> +  \nonumber \\
 &  
   \frac{1}{2} \alpha_k^2 L_1(J) \left\|  \nabla J(\bm{\theta}_k)- \bm{w}_k    \right\|^2   \geq J (\bm{\bm{\theta}}_{k}) + \alpha_k  \| {\nabla} J (\bm{\bm{\theta}}_k) \|^2 \nonumber \\
 &   - \alpha_k \bm{w}_k ^\top  \nabla J(\bm{\theta}_k)   +\frac{1}{2} \alpha_k^2 L_1(J) \left\|  \nabla J(\bm{\theta}_k)   \right\|^2 -\frac{1}{2}\alpha_k^2 L_1(J) \left\| \bm{w}_k  \right\|^2. 
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The above expression can be further expressed as 
%  \begin{align}
%&  J (\bm{\bm{\theta}}_{k}) + \alpha_k  \| {\nabla} J (\bm{\bm{\theta}}_k) \|^2- \alpha_k w_k^\top  \nabla J(\bm{\theta}_k)   +\frac{1}{2} \alpha_k^2 L_1(J) \left\|  \nabla J(\bm{\theta}_k)   \right\|^2 \nonumber \\ &-\frac{1}{2}\alpha_k^2 L_1(J) \left\|  w_k \right\|^2 \nonumber \\  \geq &  J (\bm{\bm{\theta}}_{k}) + \alpha_k  \| {\nabla} J (\bm{\bm{\theta}}_k) \|^2- \alpha_k w_k^\top  \nabla J(\bm{\theta}_k)   -\alpha_k^2 L_1(J) \left\|  w_k \right\|^2. 
% \end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
With $\alpha_k < \frac{2}{L}$  and further  simplification results in 
   \begin{align} \label{eqn_Jre}
 J(\bm{\theta}_{k+1}) \geq &  J (\bm{\bm{\theta}}_{k}) + \alpha_k  \| {\nabla} J (\bm{\bm{\theta}}_k) \|^2- \alpha_k \bm{w}_k ^\top  \nabla J(\bm{\theta}_k)   -\nonumber \\
 & \alpha_k^2 L_1(J) \left\|  \bm{w}_k  \right\|^2. 
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 Next, we need to prove that the series on the right hand side of the expression \eqref{eqn_Jre}  converges.
 We follow the similar procedure adopted in  \cite{bertsekas2000gradient}.   The following discussion summarizes the assumptions and tools used for the analysis.
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{assumption}
Let $\bm{\theta}_k$ be a sequence generated by stochastic ascent with $\alpha_k$ be the step-size. Let $ \mathcal{F}_k$ be an increasing sequence of $\sigma$- fields.  We assume the following: 
\begin{enumerate}
\item  For all  time instants $k$ and with probability 1, 
$$
\mathbb{E}\left[\bm{w}_k  |\mathcal{F}_k\right]  =0 
$$
\item For all $k$, 
$$
\mathbb{E}\left[ \|\bm{w}_k  \|^2 |\mathcal{F}_k\right]  \leq  Y_1 + Y_2 \| \nabla J(\bm{\theta}) \|^2
$$
with probability 1. 
\item We have 
$$
\sum_{t=0}^{\infty} \alpha_k =\infty, \textrm{and} \, \sum_{t=0}^{\infty} \alpha_k^2  < \infty
$$
\end{enumerate}
 \end{assumption}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{prop}{\cite{bertsekas2000gradient}} \label{prop:1} 
 Let $X_k$, $Y_k$,  and $W_k$ be three sequences  such that $W_k \geq 0, \, \forall k$. Suppose the series $\sum_{k=0}^{T} Z_k$ converges as $T \to \infty$ and $Y_{k+1} \geq Y_{k} +W_k-Z_k \, \textrm{and}  \,  |Y_k| < \infty, \, \forall k$. Then, 
 $$
 Y_k \to Y^{*} \leq \infty , \, \textrm{and} \, \sum_{k=0}^{\infty}  W_k <\infty
 $$
 \end{prop}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
As the stochastic gradients can be  unbounded,  updates either lead to  an unbounded value or a  finite objective value with $\lim_{k \to \infty}  \hat{\nabla} J(\bm{\theta}) \to 0$. The unbounded gradient here is tackled by dividing discrete time instants into two intervals, $S$ and $I$  during which $\|\nabla J(\bm{\theta}_k)\|$ is small and $\{ \tau_k, \tau_{k+1}, \ldots, \tau_{k}^{'} \} $ for which $\|\nabla J(\bm{\theta}_k)\|$ stays large, respectively.   For $k=1,2,  \, \ldots$ we define $\tau_k$ as 
 \begin{align}
 \tau_{k} = \min \{  k> \tau_{k-1}^{'}  |   \, \|\nabla J(\bm{\theta})\| \geq \delta \}.
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Let $ \delta$ be a arbitrary positive number and $\eta$  be a positive constant defined as a function of  $\delta$. It is assumed that whenever gradient is large, it stays so for sufficiently long interval  $I$ so that the objective increases atleast by a small quantity in the interval. Definition of  
 $\tau_{k}^{'}$ enforces the above assumption
 \begin{align}
&  \tau_{k}^{'} = \max \{k \geq \tau_{k} | \sum_{i =\tau_{k}}^{k} \alpha_i \leq \eta  \,   \textrm{and} \,  \nonumber \\ &  \frac{\| J(\bm{\theta}_{\tau_k})  \|}{2} \leq \| J(\bm{\theta}_{\tau_k})  \| \leq 2 \| J(\bm{\theta}_{\tau_k})  \|    \}
 \end{align}
Set, $I_{k}$ is said to be full if $\sum_{k=\tau_k}^{\tau_{k}^{'}+1} \alpha_k >\eta$. 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The above assumption helps to characterize the error in actual and stochastic gradient  in terms of  $G_k$.  For set $S$, $G_k =\delta$ and in the interval $I_k$, $G_k = \| \nabla  J(\bm{\theta}_{\tau_k})\|$, $\|\nabla J(\bm{\theta}_k) \| /G_k \leq 2$. 
% We define a  sequence $G_k$ to scale  $w_k$  as follows
%\begin{align} 
%&   \| \nabla  J(\bm{\theta}_k) \|  \nonumber \\ &= \left\{\begin{array}{lr}
%       \delta =G_k , & \text{if  }k \in  S \\
%       \frac{G_k}{2} =\frac{H_k}{2}   \leq \| \nabla J(\bm{\theta}_k) \|\leq 2 H_k  =2 G_k  &  \text{if} \, k \in I_k 
%        \end{array}\right\}
%\end{align}
%We see that the ratio of $\| J(\bm{\theta}_k)\| /G_k$ is bounded above by 2.  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 If $\tau_k$ is defined and $I_k$ is a full interval, then
$$
\frac{\eta}{2} \leq \eta -\alpha_{{\tau_{k}^{'}}+1} < \sum_{i=\tau_k}^{\tau_{k}^{'}} \alpha_i \leq \eta. 
$$  Indicator function defines  time instants  $k$  at which $\| J(\bm{\theta}_k)\|  < \delta$  expressed as 
 \[
   \chi_k = \left\{\begin{array}{lr}
       1, & \text{if  } k \in S\\
       0 & \textrm{otherwise} 
        \end{array}\right\}
  \]
is also $\mathcal{F}_k$-measurable. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{prop}{ \cite{bertsekas2000gradient}} \label{prop: finiteincre}
After a certain time, $J(\bm{\theta})$ is guaranteed to increase
by at least a constant amount during full intervals.
$$
J(\bm{\theta}_{\tau_{k}^{'}+1}) >J(\bm{\theta}_{\tau_{k}}) +h.
$$
where h is a positive constant that depends only on $\delta$.
 \end{prop}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \begin{prop}{\cite{bertsekas2000gradient}}
%There are finitely many intervals $I_k$. 
% \end{prop}
% \begin{proof}
% Results follows from Lemma 5 of \cite{bertsekas2000gradient}.
% \end{proof}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The upper bound on objective function from  Assumption \ref{Assum:Q}  along with  Proposition \ref{prop: finiteincre} rules out the possibility of infinite number of set, $I$.  Therefore, we conclude presence of only finite number of $I$. Now the above expressions along with Lemma 3 of \cite{bertsekas2000gradient}  deduce the convergent nature of right hand side of \eqref{eqn_Jre}. We elaborate it in the following discussion.  Using above definitions,  there exists a $k> k_0$ such that  $k \in S $ and indicator function $\chi_k =1$. 
%Note that $K_0$ is designed so as to satisfy Lemma 3 of \cite{bertsekas2000gradient}. 
Therefore,
 $$
 \lim_{k \to \infty} \sup \| \nabla J( \bm{\theta}_k)\| \leq \delta.
 $$  Therefore, for $k>k_0$, we get
   \begin{align}
 J (\bm{\bm{\theta}}_{k+1}) \geq &  J (\bm{\bm{\theta}}_{k}) - \chi_{k} \left\{  \alpha_k\bm{w}_k ^\top  \nabla J(\bm{\theta}_k)   + \alpha_k^2 L_1(J) \left\|  \bm{w}_k  \right\|^2\right\}. 
 \end{align}
Now following  Lemma 3 of  \cite{bertsekas2000gradient},  $\chi_{k} \left\{  \alpha_k \bm{w}_k ^\top  \nabla J(\bm{\theta}_k)   + \alpha_k^2 L_1(J) \left\| \bm{w}_k  \right\|^2\right\}$ converges. Further, using Propostion \ref{prop:1} with $W_k=0   \,  \forall k$ and $Z_k=\chi_{k} \left\{  \alpha_k \bm{w}_k ^\top  \nabla J(\bm{\theta}_k)   + \alpha_k^2 L_1(J) \left\|  \bm{w}_k  \right\|^2\right\} ,$  $J(\bm{\theta}_k)$ converges to a finite value $ J(\bm{\theta}^*)$ and $\nabla J(\bm{\theta}^*)=0$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The above result shows that the stochastic updates of \eqref{eq:policy_gradient_iteration} converges to a finite value.   Next we prove that the  policy gradients settles to a small bound in expectation. Evaluating expectation of  \eqref{eqn_Jre}, we get
   \begin{align}
\mathbb{E} \left[  J (\bm{\bm{\theta}}_{k+1}) \right]  \geq & \mathbb{E} \left[  J (\bm{\bm{\theta}}_{k}) \right] + \alpha_k  \mathbb{E} \left[  \| {\nabla} J (\bm{\bm{\theta}}_k) \|^2 \right]  \nonumber \\
&- \alpha_k^2 L_1(J)  \mathbb{E} \left[ \left\| \bm{w}_k  \right\|^2\right]. 
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  Now using the assumption on the noise sequence, $w_k$  in the above expression
  \begin{align}
& \mathbb{E} \left[  J (\bm{\bm{\theta}}_{k+1}) \right]  \geq & \mathbb{E} \left[  J (\bm{\bm{\theta}}_{k}) \right] + \alpha_k (1-L\alpha_k Y_2)  \mathbb{E} \left[  \| {\nabla} J (\bm{\bm{\theta}}_k) \|^2 \right] \nonumber \\ & - \alpha_k^2 L_1(J)  Y_1. 
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 With  $  (1-L\alpha_k Y_2) \approx 1$, 
   \begin{align}
\mathbb{E} \left[  J (\bm{\bm{\theta}}_{k+1}) \right]  \geq & \mathbb{E} \left[  J (\bm{\bm{\theta}}_{k}) \right] + \alpha_k  \mathbb{E} \left[  \| {\nabla} J (\bm{\bm{\theta}}_k) \|^2 \right]  - \alpha_k^2 L_1(J)  Y_1 
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 Rearranging the above expression yields
    \begin{align}
\mathbb{E} \left[  \| {\nabla} J (\bm{\bm{\theta}}_k) \|^2 \right]   \leq & \frac{1}{\alpha_k} \left(  \mathbb{E} \left[  J (\bm{\bm{\theta}}_{k+1}) \right] - \mathbb{E} \left[  J (\bm{\bm{\theta}}_{k}) \right]   \right)    + \alpha_k  L_1(J)  Y_1
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 Let $\bar{k} = k-k_0$, now summation on both sides from 1 to N gives, 
    \begin{align}
& \sum_{\bar{k}=1}^{N}  \mathbb{E} \left[  \| {\nabla} J (\bm{\bm{\theta}}_{\bar{k}}) \|^2 \right]   \leq  \sum_{\bar{k}=1}^{N}  \left( \frac{1}{\alpha_{\bar{k}}} -  \frac{1}{\alpha_{\bar{k}-1}} \right) \mathbb{E}  \left[  J (\bm{\bm{\theta}}_{{\bar{k}}}) \right] \nonumber \\ &+ \frac{1}{\alpha_N} \mathbb{E} \left[  J (\bm{\bm{\theta}}_{{{N+1}}}) \right]       + \frac{1}{\alpha_0} \mathbb{E} \left[  J (\bm{\bm{\theta}}_{{{0}}}) \right]  + \sum_{\bar{k}=1}^{N} \alpha_{\bar{k}} L_1(J)  Y_1
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 Now using Jenson's inequality, we get
     \begin{align}
& \sum_{\bar{k}=1}^{N}  \mathbb{E} \left[  \| {\nabla} J (\bm{\bm{\theta}}_{\bar{k}}) \|^2 \right]   \leq  \sum_{\bar{k}=1}^{N}  \left( \frac{1}{\alpha_{\bar{k}}} -  \frac{1}{\alpha_{\bar{k}-1}} \right) \mathbb{E}  \left[ | J (\bm{\bm{\theta}}_{{\bar{k}}})| \right] \nonumber \\ &+ \frac{1}{\alpha_N} \mathbb{E} \left[ | J (\bm{\bm{\theta}}_{{{N+1}}}) | \right]       + \frac{1}{\alpha_0} \mathbb{E} \left[ | J (\bm{\bm{\theta}}_{{{0}}})| \right]  + \sum_{\bar{k}=1}^{N} \alpha_{\bar{k}} L_1(J)  Y_1
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 Using upper bound of the  cost function in the above expression along with step-size $\alpha_k$ of the form $ k^{-b},  \, b \in (0,1)$, we get
      \begin{align}
\sum_{\bar{k}=1}^{N}  \mathbb{E} \left[  \| {\nabla} J (\bm{\bm{\theta}}_{\bar{k}}) \|^2 \right]   \leq & \frac{2 U_R}{\alpha_{N}(1-\gamma)} +L Y_1 + \frac{LY_1}{1-b} (N^{1-b}-1)
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Dividing the above expression throughout by $N$ and  using $\alpha_N = N^{-b} $ 
       \begin{align} 
& \frac{1}{N} \sum_{\bar{k}=1}^{N}  \mathbb{E} \left[  \| {\nabla} J (\bm{\bm{\theta}}_{\bar{k}}) \|^2 \right]   \leq & \frac{2 U_R}{(1-\gamma)}  N^{b-1} +L Y_1 + \nonumber \\ & \frac{LY_1b}{N(1-b)} (N^{1-b}-1) \label{eqn:35}
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 The above expression implies first-order convergence to a stationary point, in other words, gradient of cost function settles to a constant value  using the proposed approach with variable step-size. Expression \eqref{eqn:35} can be further used to evaluate the order of complexity of the proposed algorithm. \\
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\| \mathbf{g}_{\mu}(\bm{\theta}_k) \|^2 & = \left\|\frac{1}{1-\gamma} {\mathbb{E}_{(s,a) \sim  (1-\gamma) \rho_{\pi_{\bm{\theta}_k}}(s) \pi_{\bm{\theta}_k}  }  \left[ \hat{Q}_{\pi_{\theta}}(s,a)  \mathbb{E}_{\mathbf{u}}\left[ \frac{L_{\pi} (\bm{\bm{\theta}}+\mu \mathbf{u},s)- L_{\pi} (\bm{\bm{\theta}},s) }  {\mu} \right] \right]}\right\|^2 
%\end{align}

==> sections/old_proof.tex <==

\appendix

\subsection{Proof of Theorem \ref{main_theorem}}

The goal here is to show that the term $\frac{1}{T}\sum_{t=0}^{T-1}\|\nabla f (\bbz^t)\|^2$ decreases as $T$ increases. 
In order the start the  analysis, note that
%
\begin{align}
	\|\nabla f (\bbz^t)\|^2 \leq & 2\Big\|\frac{1}{N}\sum_{i=1}^{N} \nabla f_i (\bbz^t)-\frac{1}{N}\sum_{i=1}^{N}\nabla_{\bbx_i}\mathcal{L}_i(\bbx_i^t,\bbd_i^t,  \lambda_i^t)\Big\|^2+2\Big\|\frac{1}{N}\sum_{i=1}^{N}\nabla_{\bbx_i}\mathcal{L}_i(\bbx_i^t,\bbd_i^t,  \lambda_i^t)\Big\|^2
	\nonumber
	\\
	\leq &  \frac{2}{N}\sum_{i=1}^{N} \Big\|\nabla f_i (\bbz^t)-\nabla_{\bbx_i}\mathcal{L}_i(\bbx_i^t,\bbd_i^t,  \lambda_i^t)\Big\|^2+\frac{2}{N}\sum_{i=1}^{N}\Big\|\nabla_{\bbx_i}\mathcal{L}_i(\bbx_i^t,\bbd_i^t,  \lambda_i^t)\Big\|^2
	\nonumber
	\\
	\leq &  \frac{2}{N}\sum_{i=1}^{N} \Big\|\nabla f_i (\bbz^t)-\nabla_{\bbx_i} f_i(\bbx_i^t) -(2\lambda_i^t+1/\eta)\left(\bbx_i^t-\bbd_i^t\right) \Big\|^2+\frac{2}{N}\sum_{i=1}^{N}\Big\|\nabla_{\bbx_i}\mathcal{L}_i(\bbx_i^t,\bbd_i^t,  \lambda_i^t)\Big\|^2
	\nonumber
	\\
	\leq &  \frac{4}{N}\sum_{i=1}^{N} \Big\|\nabla f_i (\bbz^t)-\nabla_{\bbx_i} f_i(\bbx_i^t) \Big\|^2+ \frac{4(2\lambda_{\max}+1/\eta)}{N}\sum_{i=1}^{N} \|\bbx_i^t-\bbd_i^t \|^2+\frac{2}{N}\sum_{i=1}^{N}\Big\|\nabla_{\bbx_i}\mathcal{L}_i(\bbx_i^t,\bbd_i^t,  \lambda_i^t)\Big\|^2
	\nonumber
	\\
	= &  \frac{4}{N}\sum_{i=1}^{N} \Big\|\nabla f_i (\bbz^t)-\nabla_{\bbx_i} f_i(\bbx_i^t) \Big\|^2+\frac{2}{N}\sum_{i=1}^{N}\Big\|\nabla_{\bbx_i}\mathcal{L}_i(\bbx_i^t,\bbd_i^t,  \lambda_i^t)\Big\|^2
	\nonumber
	\\
	\leq &  \frac{4L^2}{N}\sum_{i=1}^{N} \|\bbz^t-\bbx_i^t \|^2+\frac{2}{N}\sum_{i=1}^{N}\Big\|\nabla_{\bbx_i}\mathcal{L}_i(\bbx_i^t,\bbd_i^t,  \lambda_i^t)\Big\|^2\label{main_2}.
\end{align}
%
Take the expectation on both sides, we get
%
\begin{align}
	\mathbb{E}[\|\nabla f (\bbz^t)\|^2 ]
	\leq &  \frac{4L^2}{N}\sum_{i=1}^{N} \mathbb{E}[\|\bbz^t-\bbx_i^t \|^2]+\frac{2}{N}\sum_{i=1}^{N}\mathbb{E}\left[\blue{\Big\|\nabla_{\bbx_i}\mathcal{L}_i(\bbx_i^t,\bbd_i^t,  \lambda_i^t)\Big\|^2}\right]\label{main_3}.
\end{align}
%

**********************************************\\
***********************************************

Let us first bound the primal gradients $\nabla_{\bbx_i}\mathcal{L}_i(\bbx_i,\bbz,  \lambda_i)$, we note that
%
\begin{align}
	\blue{	\|\nabla_{\bbx_i}\mathcal{L}_i(\bbx_i^t,\bbd_i^{t},  \lambda_i^t)\|} =& \|\nabla_{\bbx_i} f_i(\bbx_i^t) +(\lambda_i^{t}+\frac{1}{\eta})\left(\bbx_i^t-\bbd_i^{t}\right) \|\nonumber
	\\
	=& \|\nabla_{\bbx_i} f_i(\bbx_i^t) +\left(\lambda_i^{t}+\frac{1}{\eta}\right)\left(\bbx_i^t-\bbd_i^{t}\right) -\nabla f_i(\bbx_i^{t+1}) -\left(\lambda_i^{t}+\frac{1}{\eta}\right)\left(\bbx_i^{t+1}-\bbd^{t}_i\right) + \bbe_i^{t+1}\|\nonumber
	\\
	=& \|\nabla_{\bbx_i} f_i(\bbx_i^t)-\nabla f_i(\bbx_i^{t+1}) +\left(\lambda_i^{t}+\frac{1}{\eta}\right)\left(\bbx_i^t-\bbx_i^{t+1}\right)  + \bbe_i^{t+1}\|\nonumber
	\\
	\leq& L\|\bbx_i^{t+1}-\bbx_i^t\| +\left(\lambda_i^{t}+\frac{1}{\eta}\right)\|\bbx_i^{t+1}-\bbx_i^t\|  + \|\bbe_i^{t+1}\|\nonumber
	\\
	\leq& \frac{1+\eta(L+\lambda_{\max})}{\eta}\|\bbx_i^{t+1}-\bbx_i^t\|  +\sqrt{\epsilon_1}.\label{grad_x1}
\end{align}
%
Let us define $L':= L+\lambda_{\max}$ and taking the square on both sides, we get
%
\begin{align}
	\|\nabla_{\bbx_i}\mathcal{L}_i(\bbx_i^t,\bbd_i^{t},  \lambda_i^t)\|^2\leq &\left(\frac{1+\eta L'}{\eta}\right)^2\|\bbx_i^{t+1}-\bbx_i^t\|^2  +{\epsilon_1}.\label{grad_x2}
\end{align}
%
When no communication or aggregation is performed at $t$, we note that $\bbd_i^t=\bbx_i^t$, we can write
%
\begin{align}
	\nabla_{\bbz}\mathcal{L}_i(\bbx_i^t,\bbd_i^t,  \lambda_i^t) =& -(2\lambda_i^t+1/\eta)\left(\bbx_i^t-\bbd_i^t\right)=0.\label{grad_z2}
\end{align}
%
When the aggregation is performed at iteration $t$, then we have $\bbd_i^t=\frac{1}{\sum_{j=1}^{N}(\lambda_j^{t}+1/\eta) }\sum_{j=1}^{N}(\lambda_j^{t}+1/\eta)\bbx_j^{t}$
%
\begin{align}
	\nabla_{\bbz}\mathcal{L}_i(\bbx_i^t,\bbd_i^t,  \lambda_i^t) =& -\frac{1}{N}\sum_{i=1}^{N}(2\lambda_i^t+1/\eta)\left(\bbx_i^t-\frac{1}{\sum_{j=1}^{N}(\lambda_j^{t}+1/\eta) }\sum_{j=1}^{N}(\lambda_j^{t}+1/\eta)\bbx_j^{t}\right)\label{grad_z3}
	=0 .
\end{align}
%

%	Let us proceed to develop the best possible upper bound on the left hand side of \eqref{grad_z3}.  Taking the norm on the both sides in \eqref{grad_z3}, we can write
%	%
%	\begin{align}
	%		\|	\nabla_{\bbz}\mathcal{L}_i(\bbx_i^t,\bbd_i^t,  \lambda_i^t) \|\leq &(2\lambda_{\max}+1/\eta) \Big\|\frac{1}{N}\sum_{i=1}^{N}\left(\bbx_i^t-\frac{1}{\sum_{j=1}^{N}\lambda_j^{t} }\sum_{j=1}^{N}\lambda_j^{t}\bbx_j^{t}\right)\Big\|\label{grad_z4}
	%		\nonumber\\
	%		= &(2\lambda_{\max}+1/\eta) \Big\|\sum_{i=1}^{N}\frac{1}{N}\cdot\bbx_i^t-\sum_{j=1}^{N}\left(\frac{\lambda_j^{t}}{\sum_{j=1}^{N}\lambda_j^{t} }\right)\bbx_j^{t}\Big\|\nonumber
	%		\\
	%		= &(2\lambda_{\max}+1/\eta) \Big\|\sum_{i=1}^{N}\left(\frac{1}{N}-\frac{\lambda_i^{t}}{\sum_{j=1}^{N}\lambda_j^{t} }\right)\bbx_i^{t}\Big\|\nonumber
	%		\\
	%		\leq &(2\lambda_{\max}+1/\eta) \sum_{i=1}^{N}\underbrace{\Big|\frac{1}{N}-\frac{\lambda_i^{t}}{\sum_{j=1}^{N}\lambda_j^{t} }\Big|}_{\leq 2}\|\bbx_i^{t}\|\nonumber
	%		\\
	%		\leq &2(2\lambda_{\max}+1/\eta) \sum_{i=1}^{N}\underbrace{\|\bbx_i^{t}\|}_{\leq C}
	%		\nonumber
	%		\\
	%		\leq &2(2\lambda_{\max}+1/\eta) N C .
	%	\end{align}
%	%
%	
%	\red{Alternative bound, we have}
%	%
%	\begin{align}
	%		\|	\nabla_{\bbz}\mathcal{L}_i(\bbx_i^t,\bbd_i^t,  \lambda_i^t) \|
	%		\leq
	%		&(2\lambda_{\max}+1/\eta) \frac{1}{N}\sum_{i=1}^{N}\Big\|\bbx_i^t-\frac{1}{\sum_{j=1}^{N}\lambda_j^{t} }\sum_{j=1}^{N}\lambda_j^{t}\bbx_j^{t}\Big\|\label{grad_z41}
	%		\\
	%		=& (2\lambda_{\max}+1/\eta) \frac{1}{N}\sum_{i=1}^{N}\Big\|\frac{1}{\sum_{j=1}^{N}\lambda_j^{t} }\sum_{j=1}^{N}\lambda_j^{t}\bbx_i^t-\frac{1}{\sum_{j=1}^{N}\lambda_j^{t} }\sum_{j=1}^{N}\lambda_j^{t}\bbx_j^{t}\Big\|\label{grad_z422}
	%		\\
	%		=& (2\lambda_{\max}+1/\eta) \frac{1}{N}\sum_{i=1}^{N}\Big\|\frac{1}{\sum_{j=1}^{N}\lambda_j^{t} }\sum_{j=1}^{N}\lambda_j^{t}(\bbx_i^t-\bbx_j^{t})\Big\|\nonumber
	%		\\
	%		\leq  & (2\lambda_{\max}+1/\eta) \frac{1}{N}\sum_{i=1}^{N}\frac{1}{\sum_{j=1}^{N}\lambda_j^{t} }\sum_{j=1}^{N}\lambda_j^{t}\|\bbx_i^t-\bbx_j^{t}\|\nonumber
	%		\\
	%		\leq &(2\lambda_{\max}+1/\eta) \frac{1}{N}\sum_{i=1}^{N}1\cdot\|\bbx_i^t-\bbx_j^{t}\|\nonumber
	%		\\
	%		\leq &(2\lambda_{\max}+1/\eta) \frac{1}{N}\sum_{i\neq j}\|\bbx_i^t-\bbx_j^{t}\|.
	%	\end{align}
%	%
%	Taking the square root on the both sides, we get
%	%
%	\begin{align}
	%		\|	\nabla_{\bbz}\mathcal{L}_i(\bbx_i^t,\bbd_i^t,  \lambda_i^t) \|^2
	%		\leq &(2\lambda_{\max}+1/\eta)^2\sum_{i\neq j}\|\bbx_i^t-\bbx_j^{t}\|^2.\label{grad_z22}
	%	\end{align}
%	%
%	
%	Further, the gradient with respect to dual variable $\lambda$, we get
%	%
%	\begin{align}
	%		\|\nabla_{\lambda_i}\mathcal{L}_i(\bbx_i^t,\bbd_i^t,  \lambda_i^t)\|^2 =& \|h_i(\bbx_i^t,\bbd_i^t)\|^2\label{grad_lambda_2}
	%		%					
	%		%					\|\bbx_i^t-\bbd_i^{t-1}+\bbd_i^{t-1}-\bbd_i^t\|^2-\gamma_i\nonumber
	%		%					\\
	%		%					 \leq & 2\|\bbx_i^t-\bbd_i^{t-1}\|^2+2\|\bbd_i^t-\bbd_i^{t-1}\|^2-\gamma_i\nonumber
	%		%					 \\
	%		%					 = & 2\left(\|\bbx_i^t-\bbd_i^{t-1}\|^2-\gamma_i\right)+2\|\bbd_i^t-\bbd_i^{t-1}\|^2+\gamma_i
	%	\end{align}
%
%	Adding the terms \eqref{grad_x2}, \eqref{grad_z22}, and \eqref{grad_lambda_2}, we obtain
%	%
%	\begin{align}
	%		\|\nabla\mathcal{L}_i(\bbx_i^t,\bbd_i^t,  \lambda_i^t)\|^2=&\|\nabla_{\bbx_i}\mathcal{L}_i(\bbx_i^t,\bbd_i^{t},  \lambda_i^t)\|^2+\|	\nabla_{\bbz}\mathcal{L}_i(\bbx_i^t,\bbd_i^t,  \lambda_i^t) \|^2+	\|\nabla_{\lambda_i}\mathcal{L}_i(\bbx_i^t,\bbd_i^t,  \lambda_i^t)\|^2 \nonumber
	%		\\
	%		\leq &\left(\frac{1+\eta(L+\lambda_{\max})}{\eta}\right)^2\|\bbx_i^{t+1}-\bbx_i^t\|^2  +{\epsilon_1}\nonumber
	%	%	\\
	%	%	& +(2\lambda_{\max}+1/\eta)^2\sum_{i\neq j}\|\bbx_i^t-\bbx_j^{t}\|^2
	%	%	\nonumber
	%	%	\\
	%	%	&\quad
	%		+\|h_i(\bbx_i^t,\bbd_i^t)\|^2.
	%	\end{align}
%
Take expectation on both sides, then take summation over $i$, we can write
%
%
\begin{align}
	\frac{1}{N}\sum_{i=1}^{N}\mathbb{E}[\|\nabla_{\bbx_i}\mathcal{L}_i(\bbx_i^t,\bbd_i^t,  \lambda_i^t)\|^2]
	\leq &C_2\left[\frac{1}{N}\sum_{i=1}^{N}\mathbb{E}[\|\bbx_i^{t+1}-\bbx_i^t\|^2]  +{\epsilon_1}\right].\label{first_main}
\end{align}
%
where $C_2\geq \max\big\{\left(\frac{1+\eta L'}{\eta}\right)^2,1\big\}$.

********************************************************\\
********************************************************

%\begin{lemma}\label{lemma_first}
%	The Algorithm iterates generated by the FedBC satisfies
%	%
%	\begin{align}
	%	\mathcal{L}_i(\bbx_i^{t+1},\bbd_i^{t+},  \lambda_i^{t+1})-\mathcal{L}_i(\bbx_i^{t},\bbd_i^t,  \lambda_i^{t})\leq& \frac{\epsilon_1}{2L}- \left(\lambda_{\min}+\frac{1}{2\eta}- L\right)\|\bbx_i^{t+1}-\bbx_i^{t}\| ^2 + \alpha |\|\bbx_i^{t+1}-\bbd^{t}_i\|^2-\gamma_i|^2
	%\nonumber
	%\\
	%&\quad-\left(\lambda_{\min}+\frac{1}{2\eta}\right)\|\bbd^{t+}-\bbd^{t}_i\|^2.	\end{align}
	%\end{lemma}
	%%
	
	
	In order to bound the right hand side of \eqref{first_main}, let us consider the Lagrangian difference as
	%
	\begin{align}\label{main}
		\mathcal{L}_i(\bbx_i^{t+1},\bbz^{t+1},  \lambda_i^{t+1})-\mathcal{L}_i(\bbx_i^{t},\bbz^{t},  \lambda_i^{t}) =& \underbrace{\mathcal{L}_i(\bbx_i^{t+1},\bbz^{t},  \lambda_i^{t})-\mathcal{L}_i(\bbx_i^{t},\bbz^{t},  \lambda_i^{t})}_{I} \nonumber
		\\
		& \quad\underbrace{\mathcal{L}_i(\bbx_i^{t+1},\bbz^{t},  \lambda_i^{t+1})-\mathcal{L}_i(\bbx_i^{t+1},\bbz^{t},  \lambda_i^{t})}_{II}\nonumber
		\\
		&\quad\quad\underbrace{\mathcal{L}_i(\bbx_i^{t+1},\bbz^{t+1},  \lambda_i^{t+1})-\mathcal{L}_i(\bbx_i^{t+1},\bbz^{t},  \lambda_i^{t+1})}_{III}.
	\end{align}
	
	Next we establish upper bounds for the terms $I, II$ and $III$ separately as follows.
	
	\textbf{Bound on $I$:} Using the definition of the Lagrangian, we can write
	%
	\begin{align}
		I= & f_i(\bbx_i^{t+1}) +\lambda_i^{t}\left(\|\bbx_i^{t+1}-\bbz^{t}\|^2-\gamma_i\right) +\frac{1}{2\eta}\|\bbx_i^{t+1}-\bbz^{t}\|^2\nonumber
		\\
		& -f_i(\bbx_i^{t}) -\lambda_i^{t}\left(\|\bbx_i^{t}-\bbz^{t}\|^2-\gamma_i\right)-\frac{1}{2\eta}\|\bbx_i^{t}-\bbz^{t}\|^2
		\nonumber
		\\
		= & f_i(\bbx_i^{t+1})-f_i(\bbx_i^{t}) +\lambda_i^{t}\left(\|\bbx_i^{t+1}-\bbz^{t}\|^2-\|\bbx_i^{t}-\bbz^{t}\|^2\right).
	\end{align}
	%
	From the Lipschitz smoothness of the objective function, we can write
	%
	\begin{align}
		I= & \langle\nabla f_i(\bbx_i^{t+1}),\bbx_i^{t+1}-\bbx_i^{t}\rangle+ \frac{L}{2}\|\bbx_i^{t+1}-\bbx_i^{t}\| ^2\nonumber
		\\
		& +\left(\lambda_i^{t}+\frac{1}{2\eta}\right)\left(\|\bbx_i^{t+1}-\bbz^{t}\|^2-\|\bbx_i^{t}-\bbz^{t}\|^2\right).
	\end{align}
	%
	Utilizing the equality $\|\bba\|^2-\|\bbb\|^2=\langle\bba+\bbb,\bba-\bbb\rangle$, we obtain
	%
	\begin{align}
		I= & \langle\nabla f_i(\bbx_i^{t+1}),\bbx_i^{t+1}-\bbx_i^{t}\rangle+ \frac{L}{2}\|\bbx_i^{t+1}-\bbx_i^{t}\| ^2\nonumber
		\\
		& +\left(\lambda_i^{t}+\frac{1}{2\eta}\right)\left(\langle2\bbx_i^{t+1}-\bbx_i^{t+1}+\bbx_i^{t}-2\bbz^{t},\bbx_i^{t+1}-\bbx_i^{t}\rangle\right)\nonumber
		\\
		= & \langle\nabla f_i(\bbx_i^{t+1}),\bbx_i^{t+1}-\bbx_i^{t}\rangle+ \frac{L}{2}\|\bbx_i^{t+1}-\bbx_i^{t}\| ^2\nonumber
		\\
		& +2\left(\lambda_i^{t}+\frac{1}{2\eta}\right)\left(\langle\bbx_i^{t+1}-\bbz^{t},\bbx_i^{t+1}-\bbx_i^{t}\rangle\right) -\left(\lambda_i^{t}+\frac{1}{2\eta}\right)\|\bbx_i^{t+1}-\bbx_i^{t}\|^2.
	\end{align}
	%
	After rearranging the terms, we get
	%
	\begin{align}
		I= & \langle\nabla f_i(\bbx_i^{t+1})+2\left(\lambda_i^{t}+\frac{1}{2\eta}\right)(\bbx_i^{t+1}-\bbz^{t}) ,\bbx_i^{t+1}-\bbx_i^{t}\rangle+ \frac{L}{2}\|\bbx_i^{t+1}-\bbx_i^{t}\| ^2\nonumber
		\\
		& -\left(\lambda_i^{t}+\frac{1}{2\eta}\right)\|\bbx_i^{t+1}-\bbx_i^{t}\|^2.
	\end{align}
	%
	Using the Peter-Paul inequality, we obtain
	%
	\begin{align}
		I= & \frac{1}{2L}\|\nabla f_i(\bbx_i^{t+1})+2\lambda_i^{t}(\bbx_i^{t+1}-\bbz^{t})\|^2+ L\|\bbx_i^{t+1}-\bbx_i^{t}\| ^2\nonumber
		\\
		& -\left(\lambda_i^{t}+\frac{1}{2\eta}\right)\|\bbx_i^{t+1}-\bbx_i^{t}\|^2.
	\end{align}
	%
	From the optimality condition of the local oracle, we know that $\nabla f_i(\bbx_i^{t+1})+2\lambda_i^{t}(\bbx_i^{t+1}-\bbz^{t})=\bbe^{t+1}_i$, we can write
	%
	\begin{align}
		I\leq & \frac{\epsilon_1}{2L}- \left(\frac{1-2\eta L}{2\eta}\right)\|\bbx_i^{t+1}-\bbx_i^{t}\| ^2. \label{bounds_I}
	\end{align}
	%
	{We obtain a condition on $\eta$ here as $0<\eta< \frac{1}{ 2 L}$.}
	
	\textbf{Bound on $II$:} Let us consider the term $II$ after substituting the value of the Lagrangian, we get
	%
	\begin{align}
		II= & (\lambda_i^{t+1}-\lambda_i^{t})\left(\|\bbx_i^{t+1}-\bbz^{t}\|^2-\gamma_i\right). 
		\nonumber
		\\
		\leq & |\lambda_i^{t+1}-\lambda_i^{t}|\cdot |\left(\|\bbx_i^{t+1}-\bbz^{t}\|^2-\gamma_i\right)|
	\end{align}
	%
	From the update of dual variable, we can write
	\begin{align}
		II\leq  \alpha |h_i(\bbx_i^{t+1},\bbz^{t})|^2 \leq \red{\alpha G^2}.\label{bounds_II}
	\end{align}
	%
	
	\textbf{Bound on $III$:} Let us consider the term $III$ after substituting the value of the Lagrangian, we get
	
	%
	\begin{align}
		III= & \left(\lambda_i^{t+1}+\frac{1}{2\eta}\right)\left(\|\bbx_i^{t+1}-\bbz^{t+1}\|^2-\|\bbx_i^{t+1}-\bbz^{t}\|^2\right) \nonumber
		\\
		=& \left(\lambda_i^{t+1}+\frac{1}{2\eta}\right)\left( \langle2\bbx_i^{t+1}-2\bbz^{t+1}+\bbz^{t+1}-\bbz^{t},\bbz^{t} -\bbz^{t+1} \rangle\right) \nonumber
		\\
		=& 2\left(\lambda_i^{t+1}+\frac{1}{2\eta}\right)\left( \langle\bbx_i^{t+1}-\bbz^{t+1},\bbz^{t} -\bbz^{t+1} \rangle\right)
		\nonumber
		\\
		&\quad-\left(\lambda_i^{t+1}+\frac{1}{2\eta}\right)\|\bbz^{t+1}-\bbz^{t}\|^2
		\\
		\leq & \red{2\left(\lambda_{\max}+\frac{1}{2\eta}\right)\|\bbx_i^{t+1}-\bbz^{t+1}\| \|\bbz^{t}-\bbz^{t+1}\|}
	\end{align}
	%
	Next, we utilize the upper bounds on $I,II$, and $III$ into \eqref{main} to obtain
	%
	\begin{align}
		\mathcal{L}_i(\bbx_i^{t+1},\bbz^{t+1},  \lambda_i^{t+1})-\mathcal{L}_i(\bbx_i^{t},\bbz^{t},  \lambda_i^{t})\leq& \frac{\epsilon_1}{2L}- \left(\frac{1-2\eta L}{2\eta}\right)\|\bbx_i^{t+1}-\bbx_i^{t}\| ^2 + \alpha G^2\nonumber
		\\
		& + \red{2\left(\lambda_{\max}+\frac{1}{2\eta}\right)\|\bbx_i^{t+1}-\bbz^{t+1}\| \|\bbz^{t}-\bbz^{t+1}\|}
	\end{align}
	% 
	After rearranging the terms, we can write
	%%
	\begin{align}
		&\left(\frac{1-2\eta L}{2\eta}\right)\|\bbx_i^{t+1}-\bbx_i^{t}\| ^2 - \alpha G^2
		\nonumber
		\\
		&\qquad\qquad\qquad\qquad\leq  \mathcal{L}_i(\bbx_i^{t},\bbz^t,  \lambda_i^{t})-\mathcal{L}_i(\bbx_i^{t+1},\bbz^{t+1},  \lambda_i^{t+1}) +\frac{\epsilon_1}{2L}
		\nonumber
		\\
		&\hspace{3cm} + \red{2\left(\lambda_{\max}+\frac{1}{2\eta}\right)\|\bbx_i^{t+1}-\bbz^{t+1}\| \|\bbz^{t}-\bbz^{t+1}\|}
	\end{align}
	% 
	% 
	After rearranging the terms, we can write
	%%
	\begin{align}
		&\left(\frac{1-2\eta L}{2\eta}\right)\|\bbx_i^{t+1}-\bbx_i^{t}\| ^2+\frac{\epsilon_1}{2L}
		\nonumber
		\\
		&\hspace{3cm}\leq  \mathcal{L}_i(\bbx_i^{t},\bbz^{t},  \lambda_i^{t})-\mathcal{L}_i(\bbx_i^{t+1},\bbz^{t+1},  \lambda_i^{t+1}) +\frac{\epsilon_1}{L}+\alpha G^2
		\nonumber
		\\
		&\hspace{3cm} + \red{2\left(\lambda_{\max}+\frac{1}{2\eta}\right)\|\bbx_i^{t+1}-\bbz^{t+1}\| \|\bbz^{t}-\bbz^{t+1}\|}.
	\end{align}
	% 
	Take expectation and summation on both sides, we get
	%
	%%
	\begin{align}
		&\left(\frac{1-2\eta L}{2\eta}\right)\sum_{i=1}^{N}\mathbb{E}\left[\|\bbx_i^{t+1}-\bbx_i^{t}\| ^2\right] +\frac{\epsilon_1N}{2L}
		\nonumber
		\\
		&\hspace{3cm}\leq  \sum_{i=1}^{N}\mathbb{E}\left[\mathcal{L}_i(\bbx_i^{t},\bbz^{t},  \lambda_i^{t})-\mathcal{L}_i(\bbx_i^{t+1},\bbz^{t+1},  \lambda_i^{t+1})\right] +\frac{\epsilon_1N}{L}+\alpha N G^2\label{here5}
		\nonumber
		\\
		&\hspace{3cm} + \red{2\left(\lambda_{\max}+\frac{1}{2\eta}\right)\sum_{i=1}^{N}\|\bbx_i^{t+1}-\bbz^{t+1}\| \|\bbz^{t}-\bbz^{t+1}\|}
	\end{align}
	% 
	
	**********************************************\\
	**********************************************
	
	Next, substitute the upper bound from \eqref{second_main} into the \eqref{first_main} after taking expectation of , we can write
	%
	%
	%
	\begin{align}
		\frac{1}{N}\sum_{i=1}^{N}\mathbb{E}[\|\nabla_{\bbx_i}\mathcal{L}_i(\bbx_i^t,\bbd_i^t,  \lambda_i^t)\|^2]
		\leq &C_2\left[\frac{1}{N}\sum_{i=1}^{N}\mathbb{E}[\|\bbx_i^{t+1}-\bbx_i^t\|^2]  +{\epsilon_1}\right].\label{first_main222}
		\\
		\leq &\frac{C_2}{C_1}\frac{1}{N} \sum_{i=1}^{N}\mathbb{E}\left[\mathcal{L}_i(\bbx_i^{t},\bbz^t,  \lambda_i^{t})-\mathcal{L}_i(\bbx_i^{t+1},\bbz^{t+1},  \lambda_i^{t+1})\right] 	\nonumber
		\\
		&\hspace{0cm}+ 	\red{2\left(\lambda_{\max}+\frac{1}{2\eta}\right)\sum_{i=1}^{N}\|\bbx_i^{t+1}-\bbz^{t+1}\| \|\bbz^{t}-\bbz^{t+1}\|}
		\nonumber
		\\
		&\hspace{1cm}+\frac{C_2}{C_1}\frac{\epsilon_1N}{L}+\frac{C_2}{C_1}\alpha N G^2.\label{first_main2}
	\end{align}
	%
	Taking the summation over $t$, we get
	%
	\begin{align}
		\frac{1}{N}\sum_{i=1}^{N}\sum_{t=0}^{T-1}\mathbb{E}[\|\nabla_{\bbx_i}\mathcal{L}_i(\bbx_i^t,\bbd_i^t,  \lambda_i^t)\|^2]
		\leq &\frac{C_2}{C_1}\frac{1}{N} \sum_{i=1}^{N}\mathbb{E}\left[\mathcal{L}_i(\bbx_i^{0},\bbz^0,  \lambda_i^{0})-\mathcal{L}_i(\bbx_i^{T},\bbz^{T},  \lambda_i^{T})\right] 	\nonumber
		\\
		&\hspace{0cm}+ 	\frac{C_2}{C_1}p \sum_{t=0}^{T-1}\red{2\left(\lambda_{\max}+\frac{1}{2\eta}\right)\sum_{i=1}^{N}\|\bbx_i^{t+1}-\bbz^{t+1}\| \|\bbz^{t}-\bbz^{t+1}\|}
		\nonumber
		\\
		&\hspace{0cm}+\frac{C_2}{C_1}\frac{\epsilon_1N T}{L}+\frac{C_2G^2T}{C_1}\alpha.\label{first_main22}
	\end{align}
	%
	*****************************************************\\**********************************************
	
	
	Using \eqref{first_main22} into \eqref{main_3}, we get
	%
	\begin{align}
		\sum_{t=0}^{T-1}\mathbb{E}[\|\nabla f (\bbz^t)\|^2] \leq &  \frac{4L^2}{N}\sum_{t=0}^{T-1}\sum_{i=1}^{N} \mathbb{E}\left[\|\bbz^t-\bbx_i^t \|^2\right]+\frac{2}{N}\sum_{i=1}^{N}\sum_{t=0}^{T-1}\mathbb{E}[\|\nabla_{\bbx_i}\mathcal{L}_i(\bbx_i^t,\bbd_i^t,  \lambda_i^t)\|^2]
		\nonumber
		\\
		\leq &  \frac{4L^2}{N}\red{\sum_{t=0}^{T-1}\sum_{i=1}^{N} \mathbb{E}[\|\bbz^t-\bbx_i^t \|^2]}+\frac{2C_2}{C_1}\frac{1}{N} \sum_{i=1}^{N}\mathbb{E}\left[\mathcal{L}_i(\bbx_i^{0},\bbd_i^0,  \lambda_i^{0})-\mathcal{L}_i(\bbx_i^{T},\bbd_i^{T},  \lambda_i^{T})\right] 	\nonumber
		\\
		&\hspace{0cm}+ 	\frac{C_2}{C_1}p (\lambda_{\max}+{1}/{\eta}) \sum_{t=0}^{T-1}\red{2\left(\lambda_{\max}+\frac{1}{2\eta}\right)\sum_{i=1}^{N}\|\bbx_i^{t+1}-\bbz^{t+1}\| \|\bbz^{t}-\bbz^{t+1}\|}
		\nonumber
		\\
		&\hspace{0cm}+\frac{C_2}{C_1}\frac{\epsilon_1N T}{L}+\frac{C_2G^2T}{C_1}\alpha\label{new_main}
	\end{align}
	
	************************************************\\
	************************************************
	
	Let us first analyze the case when there is full communications. which means  $\bbd^{t+}_i = \bbx^{t+1}_i$ and $ \bbd^{t+}_j = \bbx^{t+1}_j$, which implies that 
	%
	%
	\begin{align}
		\sum_{t=0}^{T-1}\mathbb{E}[\|\nabla f (\bbz^t)\|^2] \leq &  \frac{4L^2}{N}\sum_{t=0}^{T-1}\sum_{i=1}^{N} \mathbb{E}\left[\|\bbz^t-\bbx_i^t \|^2\right]+\frac{2}{N}\sum_{i=1}^{N}\sum_{t=0}^{T-1}\mathbb{E}[\|\nabla_{\bbx_i}\mathcal{L}_i(\bbx_i^t,\bbd_i^t,  \lambda_i^t)\|^2]
		\nonumber
		\\
		\leq &  \frac{4L^2}{N}\red{\sum_{t=0}^{T-1}\sum_{i=1}^{N} \mathbb{E}[\|\bbz^t-\bbx_i^t \|^2]}+\frac{2C_2}{C_1}\frac{1}{N} \sum_{i=1}^{N}\mathbb{E}\left[\mathcal{L}_i(\bbx_i^{0},\bbd_i^0,  \lambda_i^{0})-\mathcal{L}_i(\bbx_i^{T},\bbd_i^{T},  \lambda_i^{T})\right] 	\nonumber
		\\
		&\hspace{0cm}+ 	\frac{C_2}{C_1}p (\lambda_{\max}+{1}/{\eta}) \sum_{t=0}^{T-1}\sum_{j\neq i}\red{\mathbb{E}\left[\|\bbx^{t+1}_i-\bbx^{t+1}_j\|^2\right]}
		\nonumber
		\\
		&\hspace{0cm}+\frac{C_2}{C_1}\frac{\epsilon_1N T}{L}+\frac{C_2G^2T}{C_1}\alpha\label{new_main22}
	\end{align}
	%
	Note that
	%
	\begin{align}
		\|\bbz^t-\bbx_i^t \|^2=&\|\bbx_i^t-\bbz^t\|^2\nonumber
		\\
		=&\Bigg\|\bbx^{t}_i-\frac{1}{\sum_{j=1}^{N}\lambda_j^{t+1} }\sum_{j=1}^{N}\lambda_j^{t+1}\bbx_j^{t}\Bigg\|^2
		\nonumber
		\\
		=&\Bigg\|\frac{1}{\sum_{j=1}^{N}\lambda_j^{t+1} }\sum_{j=1}^{N}\lambda_j^{t+1}\bbx^{t}_i-\frac{1}{\sum_{j=1}^{N}\lambda_j^{t+1} }\sum_{j=1}^{N}\lambda_j^{t+1}\bbx_j^{t}\Bigg\|^2
		\nonumber
		\\
		=&\Bigg\|\sum_{j=1}^{N}\frac{\lambda_j^{t+1}}{\sum_{j=1}^{N}\lambda_j^{t+1} } (\bbx^{t}_i-\bbx_j^{t})\Bigg\|^2	\nonumber
		\\
		\leq&\sum_{j=1}^{N}\frac{\lambda_j^{t+1}}{\sum_{j=1}^{N}}\|\bbx^{t}_i-\bbx_j^{t}\|^2\nonumber
		\\
		\leq&\sum_{j\neq i}\|\bbx^{t}_i-\bbx_j^{t}\|^2
		\nonumber
		\\
		\leq&\max_{i,j}\|\bbx^{t}_i-\bbx_j^{t}\|^2: =\triangle \bbx^t. \label{x_bound}\end{align}
	
	We start with bounding the difference $\|\bbx_i^{t+1}-\bbx_j^{t+1}\|$ for any arbitrary $i\neq j$. Before starting with the proof, note that
	%
	\begin{align}
		\nabla f_i(\bbx_i^{t+1}) +\left(\lambda_i^{t}+\frac{1}{\eta}\right)\left(\bbx_i^{t+1}-\bbd^{t}_i\right) = \bbe_i^{t+1},
	\end{align}
	%
	which implies that 
	%
	\begin{align}
		\bbx_i^{t+1}= \bbd^{t}_i+\frac{\bbe_i^{t+1}-\nabla f_i(\bbx_i^{t+1})}{\left(\lambda_i^{t}+\frac{1}{\eta}\right)}.
	\end{align}
	%
	From the above expression, we can write
	%
	\begin{align}
		\|\bbx_i^{t+1}-\bbx_j^{t+1}\|=\Bigg\| \bbd^{t}_i+\frac{\bbe_i^{t+1}-\nabla f_i(\bbx_i^{t+1})}{a_i} -  \bbd^{t}_j+\frac{\bbe_j^{t+1}-\nabla f_j(\bbx_j^{t+1})}{a_j}\Bigg\|,
	\end{align}
	%
	where $a_i:=\left(\lambda_i^{t}+\frac{1}{\eta}\right)$. After rearranging the terms and applying Cauchy-Schwartz inequality, we can write
	%
	\begin{align}
		\|\bbx_i^{t+1}-\bbx_j^{t+1}\|\leq & \| \bbd^{t}_i- \bbd^{t}_j\|+\Bigg\|\frac{\bbe_i^{t+1}-\nabla f_i(\bbx_i^{t+1})}{a_i} -\frac{\bbe_j^{t+1}-\nabla f_j(\bbx_j^{t+1})}{a_j}\Bigg\|
		\nonumber
		\\
		=& \| \bbd^{t}_i- \bbd^{t}_j\|+\frac{1}{a_ia_j}\|{a_j\bbe_i^{t+1}-a_i\bbe_j^{t+1}-a_j\nabla f_i(\bbx_i^{t+1})+a_i\nabla f_j(\bbx_j^{t+1})} \|
		\nonumber
		\\
		\leq& \| \bbd^{t}_i- \bbd^{t}_j\|+\frac{1}{a_i}\|{\bbe_i^{t+1}\|+\frac{1}{a_j}\|\bbe_j^{t+1}\|+\frac{1}{a_ia_j}\|a_j\nabla f_i(\bbx_i^{t+1})-a_i\nabla f_j(\bbx_j^{t+1})} \|.
	\end{align}
	%
	Next, note that $a_i\geq \frac{1}{\eta}$, which implies that $1/a_i\leq \eta$, hence we can write
	%
	%
	\begin{align}
		\|\bbx_i^{t+1}-\bbx_j^{t+1}\|
		\leq& \| \bbd^{t}_i- \bbd^{t}_j\|+2\eta \sqrt{\epsilon_1}+\eta^2\|a_j\nabla f_i(\bbx_i^{t+1})-a_i\nabla f_j(\bbx_j^{t+1}) \|. \label{here_1}
	\end{align}
	%
	Consider the term $\|a_j\nabla f_i(\bbx_i^{t+1})+a_i\nabla f_j(\bbx_j^{t+1}) \|$, we have
	%
	\begin{align}
		\|a_j\nabla f_i(\bbx_i^{t+1})+a_i\nabla f_j(\bbx_j^{t+1}) \|=&\|a_j(\nabla f_i(\bbx_i^{t+1})-\nabla f_i(\bbx_j^{t+1})+\nabla f_i(\bbx_j^{t+1}))-a_i\nabla f_j(\bbx_j^{t+1}) \|\nonumber\\
		\leq & a_j\|\nabla f_i(\bbx_i^{t+1})-\nabla f_i(\bbx_j^{t+1})\|+\red{\|a_j\nabla f_i(\bbx_j^{t+1})-a_i\nabla f_j(\bbx_j^{t+1}) \|}
		%	\nonumber\\
		%	\leq & a_jL\|\bbx_i^{t+1}-\bbx_j^{t+1}\|
		%	\nonumber
		%	\\
		%	&+\|a_j(\nabla f_i(\bbx_j^{t+1})-\nabla f_j(\bbx_j^{t+1}))+(a_j-a_i)\nabla f_j(\bbx_j^{t+1}) \|
		\nonumber\\
		\leq & a_jL\|\bbx_i^{t+1}-\bbx_j^{t+1}\|\red{+\delta} %+ L |\lambda_i^{t}-\lambda_j^{t}|.
		\label{here_2}
	\end{align}
	%
	Using \eqref{here_2} into \eqref{here_1} and the fact that $a_i\leq \lambda_{\max}+\frac{1}{\eta}$. , we get
	%
	\begin{align}
		\|\bbx_i^{t+1}-\bbx_j^{t+1}\|
		\leq& \| \bbd^{t}_i- \bbd^{t}_j\|+2\eta \sqrt{\epsilon_1}+\eta^2(\lambda_{\max}+\frac{1}{\eta})L\|\bbx_i^{t+1}-\bbx_j^{t+1}\|+\eta^2(\lambda_{\max}+\frac{1}{\eta})\delta%+ \eta^2L |\lambda_i^{t}-\lambda_j^{t}|
		. 
		\label{here_3}
	\end{align}
	%
	After rearranging the terms, we get
	%
	\begin{align}
		\left(1-\eta^2(\lambda_{\max}+{1}/{\eta})L\right)\|\bbx_i^{t+1}-\bbx_j^{t+1}\|
		\leq& \| \bbd^{t}_i- \bbd^{t}_j\|+2\eta \sqrt{\epsilon_1}+\eta^2(\lambda_{\max}+{1}/{\eta})\delta%+ \eta^2L |\lambda_i^{t}-\lambda_j^{t}|
		. \label{here_4}
	\end{align}
	%
	The term $C_0:=\left(1-\eta^2(\lambda_{\max}+{1}/{\eta})L\right)$ is positive if $\eta< \min\{\frac{1}{L}, \frac{1}{\lambda_{\max}}\}$.  Hence we could divide the both sides by $C_0$ to obtain
	%
	\begin{align}
		\|\bbx_i^{t+1}-\bbx_j^{t+1}\|
		\leq& \frac{\| \bbd^{t}_i- \bbd^{t}_j\|}{C_0}+\frac{2\eta \sqrt{\epsilon_1}}{C_0}+\frac{\eta^2(\lambda_{\max}+{1}/{\eta})\delta}{C_0}%+ \frac{\eta^2L |\lambda_i^{t}-\lambda_j^{t}|}{C_0}
		\nonumber
		\\
		\leq& \frac{\| \bbd^{t}_i- \bbd^{t}_j\|}{C_0}+\frac{2\eta \sqrt{\epsilon_1}}{C_0}+\frac{\eta^2(\lambda_{\max}+{1}/{\eta})\delta}{C_0}%+ + \frac{\eta^2L |\lambda_i^{t}-\lambda_j^{t}|}{C_0}
		. \label{here_5}
	\end{align}
	%
	For the full communication settings, we have $\bbd_i^{t}=\bbd_j^{t}$ for each $t$, therefore we obtain
	%
	%
	\begin{align}
		\|\bbx_i^{t+1}-\bbx_j^{t+1}\|
		\leq& \frac{2\eta \sqrt{\epsilon_1}}{C_0}+\frac{\eta^2(\lambda_{\max}+{1}/{\eta})\delta}{C_0}%+ \frac{\eta^2L |\lambda_i^{t}-\lambda_j^{t}|}{C_0}
		. \label{here_5}
	\end{align}
	%
	Since the above bound holds for any $i,j$, it would also hold for the maximum, therefor we can write the upper bound in \eqref{x_bound} as
	%
	%
	\begin{align}
		\|\bbz^t-\bbx_i^t \|^2	\leq&\max_{i,j}\|\bbx^{t}_i-\bbx_j^{t}\|^2\nonumber
		\\
		\leq& \frac{12\eta^2 {\epsilon_1}}{C_0^2}+\frac{3\eta^4(\lambda_{\max}+{1}/{\eta})^2\delta^2}{C_0^2}%+ \frac{12\eta^4L^2|\lambda_i^{t}-\lambda_j^{t}|^2}{C_0^2}
		.
		\label{x_bound2}
	\end{align}
	%
	Utilizing the upper bound in \eqref{x_bound2} to the right hand side of \eqref{new_main}, we get
	%
	%
	\begin{align}
		\frac{1}{T}\sum_{t=0}^{T-1}\mathbb{E}[\|\nabla f (\bbz^t)\|^2] 
		\leq &  \frac{48\eta^2 L^2{\epsilon_1}}{C_0^2}+\frac{12L^2\eta^4(\lambda_{\max}+{1}/{\eta})^2\delta^2}{C_0^2}%+ 	\frac{1}{T}\sum_{t=0}^{T-1}\frac{48 L^2\eta^4L|\lambda_i^{t}-\lambda_j^{t}|^2}{C_0^2}
		\nonumber
		\\
		&\hspace{0cm}+\frac{C_2}{C_1}\frac{\epsilon_1N }{L}+\frac{C_2G^2}{C_1}
		\nonumber
		\\
		&+\frac{2C_2}{C_1}\frac{1}{N} \sum_{i=1}^{N}\mathbb{E}\blue{\left[\mathcal{L}_i(\bbx_i^{0},\bbd_i^0,  \lambda_i^{0})-\mathcal{L}_i(\bbx_i^{T},\bbd_i^{T},  \lambda_i^{T})\right]} \alpha
		\label{new_main2}
	\end{align}
	%
	
	*********************************************\\
	*********************************************
	
	From the initial conditions we have $\mathcal{L}_i(\bbx_i^{0},\bbd_i^0,  \lambda_i^{0})= f_i(\bbz^0) $. Now we need a lower bound on $\mathcal{L}_i(\bbx_i^{T},\bbd_i^{T},  \lambda_i^{T})$, since we are doing full communications, we have  $\bbd_i^T=\bbz^T$, we can write 
	from the definition of Lagrangian
	%
	\begin{align}
		\mathcal{L}_i(\bbx_i^{T},\bbz^{T},  \lambda_i^{T}) =&	f_i(\bbx_i^{T})+ \lambda_i^{T}\left(\|\bbx_i^{T}-\bbz^{T}\|^2-\gamma_i\right) +\frac{1}{2\eta}\|\bbx_i^{T}-\bbz^{T}\|^2
		\nonumber
		\\
		f_i(\bbx_i^{T})=&\mathcal{L}_i(\bbx_i^{T},\bbz^{T},  \lambda_i^{T})- \lambda_i^{T}\left(\|\bbx_i^{T}-\bbz^{T}\|^2-\gamma_i\right) -\frac{1}{2\eta}\|\bbx_i^{T}-\bbz^{T}\|^2
		\nonumber
		\\
		=&\mathcal{L}_i(\bbx_i^{T},\bbz^{T},  \lambda_i^{T}){- \lambda_i^{T}\|\bbx_i^{T}-\bbz^{T}\|^2} + \gamma_i\lambda_i^{T} {-\frac{1}{2\eta}\|\bbx_i^{T}-\bbz^{T}\|^2}	\label{lagrangian_2}.
	\end{align}
	%
	From the smoothness condition, note that
	%
	%
	\begin{align}
		f_i(\bbz^T)\leq f_i(\bbx_i^T)+\langle\nabla f_i(\bbx_i^T),\bbz^T-\bbx_i^T\rangle +\frac{L}{2} \|\bbz^T-\bbx_i^T\|^2. \label{bound}
	\end{align}
	%
	Substitute the value in \eqref{lagrangian_2} into \eqref{bound}, we get
	%
	\begin{align}
		f_i(\bbz^T)\leq& \mathcal{L}_i(\bbx_i^{T},\bbz^{T},  \lambda_i^{T}){- \lambda_i^{T}\|\bbx_i^{T}-\bbz^{T}\|^2} + \gamma_i\lambda_i^{T} {-\frac{1}{2\eta}\|\bbx_i^{T}-\bbz^{T}\|^2}	
		\nonumber
		\\
		&+\langle\nabla f_i(\bbx_i^T),\bbz^T-\bbx_i^T\rangle +\frac{L}{2} \|\bbz^T-\bbx_i^T\|^2	\nonumber
		\\
		\leq& \mathcal{L}_i(\bbx_i^{T},\bbz^{T},  \lambda_i^{T}){- \lambda_i^{T}\|\bbx_i^{T}-\bbz^{T}\|^2} + \gamma_i\lambda_i^{T} {-\frac{1}{2\eta}\|\bbx_i^{T}-\bbz^{T}\|^2}	
		\nonumber
		\\
		&+\frac{G^2}{2L}+ \frac{L}{2}\|\bbz^T-\bbx_i^T\|^2+\frac{L}{2} \|\bbz^T-\bbx_i^T\|^2
		\nonumber
		\\
		\leq& \mathcal{L}_i(\bbx_i^{T},\bbz^{T},  \lambda_i^{T}){- \lambda_i^{T}\|\bbx_i^{T}-\bbz^{T}\|^2} + \gamma_i\lambda_i^{T} {-\frac{1-2\eta L}{2\eta}\|\bbx_i^{T}-\bbz^{T}\|^2}+\frac{G^2}{2L}. \label{bound2}
	\end{align}
	%
	Dropping the negative terms from the right hand side, we get
	%
	\begin{align}
		f_i(\bbz^T)
		\leq& \mathcal{L}_i(\bbx_i^{T},\bbz^{T},  \lambda_i^{T}) + \gamma_i\lambda_i^{T} +\frac{G^2}{2L}. \label{bound3}
	\end{align}
	%
	After rearranging the terms, we get
	%
	\begin{align}
		\mathcal{L}_i(\bbx_i^{T},\bbz^{T},  \lambda_i^{T})	
		\geq& f_i(\bbz^T) - \gamma_i\lambda_i^{T} -\frac{G^2}{2L}. \label{bound4}
	\end{align}
	%
	Multiply both sides by $-1$, we get
	%
	\begin{align}
		-\mathcal{L}_i(\bbx_i^{T},\bbz^{T},  \lambda_i^{T})	
		\leq& -f_i(\bbz^T) + \gamma_i\lambda_i^{T} +\frac{G^2}{2L}. \label{bound5}
	\end{align}
	%
	Add $\mathcal{L}_i(\bbx_i^{0},\bbd_i^0,  \lambda_i^{0})= f_i(\bbz^0) $ to both sides, we get
	%
	\begin{align}
		\mathcal{L}_i(\bbx_i^{0},\bbd_i^0,  \lambda_i^{0})	-\mathcal{L}_i(\bbx_i^{T},\bbz^{T},  \lambda_i^{T})	
		\leq& f_i(\bbz^0) -f_i(\bbz^T) + \gamma_i\lambda_i^{T} +\frac{G^2}{2L}. \label{bound6}
	\end{align}
	%
	%
	Next, it holds that $-f_i(\bbz^T)\leq -f_i(\bbz^\star)$, we can write
	%
	\begin{align}
		\mathcal{L}_i(\bbx_i^{0},\bbd_i^0,  \lambda_i^{0})	-\mathcal{L}_i(\bbx_i^{T},\bbz^{T},  \lambda_i^{T})	
		\leq& f_i(\bbz^0) -f_i(\bbz^\star) + \gamma_i\lambda_{\max} +\frac{G^2}{2L}. \label{bound7}
	\end{align}
	%
	Let us define the constant $B_0:=f_i(\bbz^0) -f_i(\bbz^\star) + \gamma_i\lambda_{\max} +\frac{G^2}{2L}$, we can upper bound the right hand side of \eqref{new_main2} as 
	%%
	%%
	%\begin{align}
	%	\sum_{t=0}^{T-1}\mathbb{E}[\|\nabla f (\bbz^t)\|^2] 
	%	\leq &   \frac{48\eta^2 L^2{\epsilon_1}}{C_0^2}+\frac{12L^2\eta^4(\lambda_{\max}+{1}/{\eta})^2\delta^2}{C_0^2}+ \frac{48 L^2\eta^4L|\lambda_i^{t}-\lambda_j^{t}|^2}{C_0^2}
	%	\nonumber
	%	\\
	%	&+\frac{2C_2B0}{C_1}+\frac{C_2}{C_1}\frac{\epsilon_1N T}{L}+\frac{C_2G^2T}{C_1}\alpha\label{new_main3}
	%\end{align}
	%%
	%Divide both sides by $T$, we get
	%
	\begin{align}
		\frac{1}{T}\sum_{t=0}^{T-1}\mathbb{E}[\|\nabla f (\bbz^t)\|^2] 
		= &  \frac{48\eta^2 L^2{\epsilon_1}}{C_0^2}+\frac{12L^2\eta^4(\lambda_{\max}+{1}/{\eta})^2\delta^2}{C_0^2}%+ 	\frac{1}{T}\sum_{t=0}^{T-1}\frac{48 L^2\eta^4L|\lambda_i^{t}-\lambda_j^{t}|^2}{C_0^2}
		\nonumber
		\\
		&\hspace{0cm}+\frac{C_2}{C_1}\frac{\epsilon_1N }{L} +\frac{2C_2B0}{C_1 T}+\frac{C_2G^2}{C_1}\alpha
		\label{new_main35}
	\end{align}
	%
	Next, in the order notation, we could write
	%
	\begin{align}
		\frac{1}{T}\sum_{t=0}^{T-1}\mathbb{E}[\|\nabla f (\bbz^t)\|^2] 
		= & \mathcal{O}\left(\frac{B_0}{T}\right)+ \mathcal{O}(\epsilon_1)+ \mathcal{O}(\delta^2)+ \mathcal{O}(\alpha) %+\red{	\frac{1}{T}\sum_{t=0}^{T-1}\frac{48 L^2\eta^4L|\lambda_i^{t}-\lambda_j^{t}|^2}{C_0^2}}
		\label{new_main36}
	\end{align}
	%
	%
	%%
	%%
	%\begin{align}
	%	\nabla f_i(\bbx_i^{T}) +\left(\lambda_i^{T-1}+\frac{1}{\eta}\right)\left(\bbx_i^{t+1}-\bbd^{t}_i\right) = \bbe_i^{t+1},
	%\end{align}
	%%
	
	
	
	***********************************************\\
	***********************************************
	
	Let us consider the update for $\lambda_i^{t+1}$ and $\lambda_j^{t+1}$, we can write
	%
	%\begin{align}
	%	\|\lambda_i^{t+1}-\lambda_j^{t+1}\|^2\leq& \|\lambda_i^{t}+\alpha (\nabla \mathcal{L}_i(\bbz^t, \bbx_i^{t+1}, \lambda_i^t))- \lambda_j^{t}-\alpha(\nabla \mathcal{L}_j(\bbz^t, \bbx_j^{t+1}, \lambda_j^t))\|^2
	%	\nonumber
	%	\\
	%	=& \|\lambda_i^{t} - \lambda_j^{t}+\alpha(\nabla \mathcal{L}_i(\bbz^t, \bbx_i^{t+1}, \lambda_i^t)-\nabla \mathcal{L}_j(\bbz^t, \bbx_j^{t+1}, \lambda_j^t))\|^2\nonumber
	%	\\
	%	=& \|\lambda_i^{t}- \lambda_j^{t}\|^2+\alpha^2\|\nabla \mathcal{L}_i(\bbz^t, \bbx_i^{t+1}, \lambda_i^t)-\nabla \mathcal{L}_j(\bbz^t, \bbx_j^{t+1}, \lambda_j^t)\|^2
	%	\nonumber
	%	\\
	%	&-\alpha\langle\lambda_i^{t}- \lambda_j^{t},\nabla \mathcal{L}_i(\bbz^t, \bbx_i^{t+1}, \lambda_i^t)-\nabla \mathcal{L}_j(\bbz^t, \bbx_j^{t+1}, \lambda_j^t)\rangle
	%\end{align}
	%%
	%Next, we bound the difference between $\bbd_i^{t+1}$ and $\bbd_j^{t+1}$. Note that with probability $1-p$, the communication is performed and hence we have $\bbd_i^{t+1}=\bbd_j^{t+1}$. But with probability $p$, we can write 
	%%
	%\begin{align}
	%	\mathbb{E}_{t+1}\left[\|\bbd_i^{t+1}-\bbd_j^{t+1}\|\right]= p\|\bbx_i^{t+1}-\bbx_j^{t+1}\|.\label{here_6}
	%\end{align}
	%%
	%From \eqref{here_5}, we ca write
	%%
	%\begin{align}
	%	\mathbb{E}_{t+1}\left[\|\bbd_i^{t+1}-\bbd_j^{t+1}\|\right]\leq& \frac{p\| \bbd^{t}_i- \bbd^{t}_j\|}{\left(1-\eta^2(\lambda_{\max}+{1}/{\eta})L\right)}+\frac{2p\eta \sqrt{\epsilon_1}}{\left(1-\eta^2(\lambda_{\max}+{1}/{\eta})L\right)}+\frac{\eta^2p(\lambda_{\max}+{1}/{\eta})\delta}{\left(1-\eta^2(\lambda_{\max}+{1}/{\eta})L\right)}
	%	\nonumber
	%	\\
	%	&+ \frac{2p\eta^2L\lambda_{\max}}{\left(1-\eta^2(\lambda_{\max}+{1}/{\eta})L\right)}.\label{here_7}
	%\end{align}
	%%
	%
	%Finally, stacking \eqref{here_5} and \eqref{here_7} together, we obtain
	%%
	%%
	%\begin{align}
	%	\|\bbx_i^{t+1}-\bbx_j^{t+1}\|
	%	\leq& \frac{\| \bbd^{t}_i- \bbd^{t}_j\|}{\left(1-\eta^2(\lambda_{\max}+{1}/{\eta})L\right)}+\frac{2\eta \sqrt{\epsilon_1}}{\left(1-\eta^2(\lambda_{\max}+{1}/{\eta})L\right)}+\frac{\eta^2(\lambda_{\max}+{1}/{\eta})\delta}{\left(1-\eta^2(\lambda_{\max}+{1}/{\eta})L\right)}
	%	\nonumber
	%	\\
	%	&+ \frac{2\eta^2L\lambda_{\max}}{\left(1-\eta^2(\lambda_{\max}+{1}/{\eta})L\right)}\nonumber
	%	\\
	%	\mathbb{E}_{t+1}\left[\|\bbd_i^{t+1}-\bbd_j^{t+1}\|\right]\leq& \frac{p\| \bbd^{t}_i- \bbd^{t}_j\|}{\left(1-\eta^2(\lambda_{\max}+{1}/{\eta})L\right)}+\frac{2p\eta \sqrt{\epsilon_1}}{\left(1-\eta^2(\lambda_{\max}+{1}/{\eta})L\right)}+\frac{\eta^2p(\lambda_{\max}+{1}/{\eta})\delta}{\left(1-\eta^2(\lambda_{\max}+{1}/{\eta})L\right)}
	%	\nonumber
	%	\\
	%	&+ \frac{2p\eta^2L\lambda_{\max}}{\left(1-\eta^2(\lambda_{\max}+{1}/{\eta})L\right)}.\label{here_8}
	%\end{align}
	%%
	%
	%
	%
	%
	%%Taking the absolute value on both sides and applying triangle inequality, we can write
	%%Further, the gradient with respect to dual variable $\lambda$, we get
	%%%
	%%\begin{align}
	%%	|\nabla_{\lambda_i}\mathcal{L}_i(\bbx_i^t,\bbd_i^t,  \lambda_i^t)|
	%%	\leq & 2|\left(\|\bbx_i^t-\bbd_i^{t-1}\|^2-\gamma_i\right)|+2\|\bbd_i^t-\bbd_i^{t-1}\|^2+\gamma_i
	%%	\nonumber
	%%	\\
	%%		\leq & 2|\lambda_i^t-\lambda_i^{t-1}|+2\|\bbd_i^t-\bbd_i^{t-1}\|^2+\gamma_i
	%%			\nonumber
	%%		\\
	%%		\leq & \red{4\lambda_{\max}}+2\|\bbd_i^t-\bbd_i^{t-1}\|^2+\gamma_i
	%%\end{align}
	%%Taking the absolute value on both sides and applying triangle inequality, we can write
	%%
	%
	
	


==> sections/pg_convergence.tex <==
%!TEX root = main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Following discussion establishes the convergence of this exploratory policies to first-order stationary points. First we establish convergence of the proposed policy class  without adaptive variance and then we extend it to  exploratory search with adaptive variance.  
\section{Convergence Analysis} \label{sec:convergence}
First we state the assumptions and notions used in the paper. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Assumptions}
\begin{assumption} \label{Assum:Q}
The reward function, $R$ and the parameterized policy, $\pi_{\bm{\theta}}$ satisfies the 
following properties:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{enumerate}
\item The absolute value of the reward is uniformly bounded,
$$
\sup_{(s,a) \in \mathcal{S} \times \mathcal{A}} |R(s,a)|  \leq  U_R, U_R < \infty.
$$
\item For all $ \, \bm{\bm{\theta}}_1, \, \bm{\theta}_2 \in \mathbb{R}^p$, the continuous policy, $\pi_{\bm{\theta}}$  is such that
 $\pi_{\bm{\theta}} \in \mathcal{C}^{1,1}$
\begin{align}
& | \pi_{\bm{\bm{\theta}}_1}(\cdot|s)  - \pi_{\bm{\bm{\theta}}_2}(\cdot|s )| \leq L_0(\pi) \|\bm{\bm{\theta}}_1-\bm{\bm{\theta}}_2\|, \label{eqn:c0}
\\
& \| \nabla \pi_{\bm{\bm{\theta}}_1}(\cdot|s)  - \nabla \pi_{\bm{\bm{\theta}}_2}(\cdot|s ) \| \leq L_1 (\pi) \|\bm{\bm{\theta}}_1-\bm{\bm{\theta}}_2\|.    \label{eqn:c1}
\end{align}
\end{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The direct consequence of condition 1 is a bounded Q-function given by $U_{R}/(1-\gamma)$ which implies  bounded norm on $J(\bm{\theta})$  as well.
\end{assumption}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 We define  $L_{\pi}(\bm{\theta},s) \in \mathcal{C}^{1,1}$
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align} \label{Eqn:bL}
|L_{\pi}(\bm{\theta}_1,s)-L_{\pi}(\bm{\theta}_2,s)| \leq L_0(L_{\pi}) \|\bm{\theta}_1 -\bm{\theta}_2\|.
\end{align}
\begin{align} \label{Eqn:bL1}
\|\nabla L_{\pi}(\bm{\theta}_1,s)-\nabla L_{\pi}(\bm{\theta}_2,s) \| \leq L_1(L_{\pi}) \|\bm{\theta}_1 -\bm{\theta}_2\|.
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 Now the  policy gradient can be expressed as 
\begin{align} \label{Eqn:grad_j1}
&{\nabla} _{\bm{\theta}} J_{\mu}(\bm{\theta})  = \frac{1}{(1-\gamma)} \sum_{s} (1-\gamma)  \rho_{\pi_{\bm{\theta}}}(s) \nonumber \\ 
&  \mathbb{E}_{a \sim \pi_{\bm{\theta}}(\cdot|s)} \left[ \hat{Q}_{\pi_{\bm{\theta}}}(s,a)  \nabla_{\bm{\theta}} \log \pi_{\bm{\theta}}(a|s) \right].  
\end{align} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 The update of the policy parameters is similar to stochastic gradient ascent and we can adopt  non-convex stochastic setting to analyze convergence  to first-order stationary point. 
%
\begin{definition}{(First-order stationary points)}  \label{def:1}
For a twice differentiable objective function  ${J} : \mathbb{R}^d \to  \mathbb{R}$, we say that $\bm{\theta}$ is an $\epsilon$ first order stationary point (FOSP) if 
\begin{align}
\|\nabla J(\bm{\theta}) \|  < \epsilon.
\end{align} 
\end{definition}
Next, we look into the convergence guarantees of the above approach to first-order stationary point.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{assumption}
The estimate of stochastic gradient satisfies the following assumption,
\begin{align}
\mathbb{E} \left[ \| \hat{\nabla} J(\bm{\theta}) \|^2  \right] \leq m +n \|\nabla J( \bm{\theta}) \|^2
\end{align}
\end{assumption}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Another immediate consequence of the above assumption is 
\begin{align}
\mathbb{E} \left[ \bm{w}_k |\mathcal{F}_k   \right] = & 0\\
\mathbb{E} \left[ \|\bm{w}_k\|^2 |\mathcal{F}_k   \right] = & Y_1 +Y_2 \|\nabla J(\bm{\theta}_k)\|^2, \, Y_1, Y_2>0
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Let us start the analysis by re-writing  the stochastic gradient updated as  approximate gradient estimate  as %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}\label{udpate11}
\bm{\theta}_{k+1} =  & \bm{\theta}_k  +\alpha_k \hat{ \nabla} J(\bm{\theta}_k)
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where, $\hat{ \nabla} J(\bm{\theta}_k)$ is the stochastic estimate of the true gradient ${ \nabla} J(\bm{\theta}_k)$ at $\bm{\theta}_k$. We note that the update for $\bm{\theta}_k$ in \eqref{udpate11} can be equivalently written as 
%
\begin{align}\label{optimization_problem}
\bm{\theta}_{k+1} = \argmin_{\bm{\theta} } J(\bm{\theta}_{k} )+\langle{ \nabla} J(\bm{\theta}_k),\bm{\theta}-\bm{\theta}_k\rangle+\frac{1}{2\alpha_k}\|\bm{\theta}-\bm{\theta}_k\|^2.
\end{align}
%
 We can obtain the update in \eqref{udpate11} from the optimality of unconstrained optimization in \eqref{optimization_problem}. In a more general setting, the last term $\|\bm{\theta}-\bm{\theta}_k\|^2$ could be replaced by the Bregman divergence term. The first two terms in the objective of \eqref{optimization_problem} is nothing but the first order approximation of the non-convex objective $J(\bm\theta)$ at $\bm\theta_k$. In order to incorporate the local geometrical structure [\textcolor{red}{might require some more motivation}], we proposed to use the quadratic lower bound provided by the Lipchitz property of the objective, which implies that
 %
 J

$w_k$ is the noise in the estimate. Using Taylors series expansion along with  Lipschitz smoothness of $J$,  we get
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
 J (\bm{\bm{\theta}}_{k+1}) \geq &  J (\bm{\bm{\theta}}_{k}) +  \left<{\nabla} J (\bm{\bm{\theta}}_k), \bm{\theta}_{k+1} -\bm{\theta}_{k} \right> - 
   \frac{1}{2} \alpha_k^2 L_1(J) \left\|  \bm{\theta}_{k+1} -  \bm{\theta}_{k}    \right\|^2. 
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Now using the expression from \eqref{eqn:est}, we get
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
& J (\bm{\bm{\theta}}_{k}) +  \left<{\nabla} J (\bm{\bm{\theta}}_k), \bm{\theta}_{k+1} -\bm{\theta}_{k} \right> - 
   \frac{1}{2} \alpha_k^2 L_1(J) \left\|  \bm{\theta}_{k+1} -  \bm{\theta}_{k}    \right\|^2 \geq  \nonumber \\ &  J (\bm{\bm{\theta}}_{k}) + \alpha_k \left<{\nabla} J (\bm{\bm{\theta}}_k), \nabla J(\bm{\theta}_k)- \bm{w}_k  \right> +
 \nonumber \\ &  \frac{1}{2} \alpha_k^2 L_1(J) \left\|  \nabla J(\bm{\theta}_k)-\bm{w}_k    \right\|^2. 
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Using triangular  inequality for norms, the above expression simplifies to 
 \begin{align}
&  J (\bm{\bm{\theta}}_{k}) + \alpha_k \left<{\nabla} J (\bm{\bm{\theta}}_k), \nabla J(\bm{\theta}_k)- \bm{w}_k   \right> +  \nonumber \\
 &  
   \frac{1}{2} \alpha_k^2 L_1(J) \left\|  \nabla J(\bm{\theta}_k)- \bm{w}_k    \right\|^2   \geq J (\bm{\bm{\theta}}_{k}) + \alpha_k  \| {\nabla} J (\bm{\bm{\theta}}_k) \|^2 \nonumber \\
 &   - \alpha_k \bm{w}_k ^\top  \nabla J(\bm{\theta}_k)   +\frac{1}{2} \alpha_k^2 L_1(J) \left\|  \nabla J(\bm{\theta}_k)   \right\|^2 -\frac{1}{2}\alpha_k^2 L_1(J) \left\| \bm{w}_k  \right\|^2. 
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The above expression can be further expressed as 
%  \begin{align}
%&  J (\bm{\bm{\theta}}_{k}) + \alpha_k  \| {\nabla} J (\bm{\bm{\theta}}_k) \|^2- \alpha_k w_k^\top  \nabla J(\bm{\theta}_k)   +\frac{1}{2} \alpha_k^2 L_1(J) \left\|  \nabla J(\bm{\theta}_k)   \right\|^2 \nonumber \\ &-\frac{1}{2}\alpha_k^2 L_1(J) \left\|  w_k \right\|^2 \nonumber \\  \geq &  J (\bm{\bm{\theta}}_{k}) + \alpha_k  \| {\nabla} J (\bm{\bm{\theta}}_k) \|^2- \alpha_k w_k^\top  \nabla J(\bm{\theta}_k)   -\alpha_k^2 L_1(J) \left\|  w_k \right\|^2. 
% \end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
With $\alpha_k < \frac{2}{L}$  and further  simplification results in 
   \begin{align} \label{eqn_Jre}
 J(\bm{\theta}_{k+1}) \geq &  J (\bm{\bm{\theta}}_{k}) + \alpha_k  \| {\nabla} J (\bm{\bm{\theta}}_k) \|^2- \alpha_k \bm{w}_k ^\top  \nabla J(\bm{\theta}_k)   -\nonumber \\
 & \alpha_k^2 L_1(J) \left\|  \bm{w}_k  \right\|^2. 
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 Next, we need to prove that the series on the right hand side of the expression \eqref{eqn_Jre}  converges.
 We follow the similar procedure adopted in  \cite{bertsekas2000gradient}.   The following discussion summarizes the assumptions and tools used for the analysis.
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{assumption}
Let $\bm{\theta}_k$ be a sequence generated by stochastic ascent with $\alpha_k$ be the step-size. Let $ \mathcal{F}_k$ be an increasing sequence of $\sigma$- fields.  We assume the following: 
\begin{enumerate}
\item  For all  time instants $k$ and with probability 1, 
$$
\mathbb{E}\left[\bm{w}_k  |\mathcal{F}_k\right]  =0 
$$
\item For all $k$, 
$$
\mathbb{E}\left[ \|\bm{w}_k  \|^2 |\mathcal{F}_k\right]  \leq  Y_1 + Y_2 \| \nabla J(\bm{\theta}) \|^2
$$
with probability 1. 
\item We have 
$$
\sum_{t=0}^{\infty} \alpha_k =\infty, \textrm{and} \, \sum_{t=0}^{\infty} \alpha_k^2  < \infty
$$
\end{enumerate}
 \end{assumption}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{prop}{\cite{bhatt2019policy}} \label{prop:1} 
 Let $X_k$, $Y_k$,  and $W_k$ be three sequences  such that $W_k \geq 0, \, \forall k$. Suppose the series $\sum_{k=0}^{T} Z_k$ converges as $T \to \infty$ and $Y_{k+1} \geq Y_{k} +W_k-Z_k \, \textrm{and}  \,  |Y_k| < \infty, \, \forall k$. Then, 
 $$
 Y_k \to Y^{*} \leq \infty , \, \textrm{and} \, \sum_{k=0}^{\infty}  W_k <\infty
 $$
 \end{prop}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We  partition discrete time instants into  sets, $S$ and $I$  during which $\|\nabla J(\bm{\theta}_k)\|$ is small and $\{ \tau_k, \tau_{k+1}, \ldots, \tau_{k}^{'} \} $ for which $\|\nabla J(\bm{\theta}_k)\|$ stays large, respectively.  For $k=1,2,  \, \ldots$ we define $\tau_k$ as 
 \begin{align}
 \tau_{k} = \min \{  k> \tau_{k-1}^{'}  |   \, \|\nabla J(\bm{\theta})\| \geq \delta \}.
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Let $ \delta$ be a arbitrary positive number and $\eta$  be a positive constant defined as a function of  $\delta$. Similarly, 
 $\tau_{k}^{'}$ is defined by
 \begin{align}
&  \tau_{k}^{'} = \max \{k \geq \tau_{k} | \sum_{i =\tau_{k}}^{k} \alpha_i \leq \eta  \,   \textrm{and} \,  \nonumber \\ &  \frac{\| J(\bm{\theta}_{\tau_k})  \|}{2} \leq \| J(\bm{\theta}_{\tau_k})  \| \leq 2 \| J(\bm{\theta}_{\tau_k})  \|    \}
 \end{align}
 Set, $I_{k}$ is said to be full if $\sum_{k=\tau_k}^{\tau_{k}^{'}+1} \alpha_k >\eta$. 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% We define a  sequence $G_k$ to scale  $w_k$  as follows
%\begin{align} 
%&   \| \nabla  J(\bm{\theta}_k) \|  \nonumber \\ &= \left\{\begin{array}{lr}
%       \delta =G_k , & \text{if  }k \in  S \\
%       \frac{G_k}{2} =\frac{H_k}{2}   \leq \| \nabla J(\bm{\theta}_k) \|\leq 2 H_k  =2 G_k  &  \text{if} \, k \in I_k 
%        \end{array}\right\}
%\end{align}
%We see that the ratio of $\| J(\bm{\theta}_k)\| /G_k$ is bounded above by 2.  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 If $\tau_k$ is defined and $I_k$ is a full interval, then
$$
\frac{\eta}{2} \leq \eta -\alpha_{{\tau_{k}^{'}}+1} < \sum_{i=\tau_k}^{\tau_{k}^{'}} \alpha_i \leq \eta 
$$  Indicator function  expressed as 
 \[
   \chi_k = \left\{\begin{array}{lr}
       1, & \text{if  } k \in S\\
       0 & \textrm{otherwise} 
        \end{array}\right\}
  \]
is also $\mathcal{F}_k$-measurable. Without loss of generality, we  assume that the above condition hold for all $k$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{prop}{ \cite{bertsekas2000gradient}}
After a certain time, $J(\bm{\theta})$ is guaranteed to increase
by at least a constant amount during full intervals.
$$
J(\bm{\theta}_{\tau_{k}^{'}+1}) >J(\bm{\theta}_{\tau_{k}}) +h.
$$
where h is a positive constant that depends only on $\delta$.
 \end{prop}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{prop}{\cite{bertsekas2000gradient}}
There are finitely many intervals $I_k$. 
 \end{prop}
 \begin{proof}
 Results follows from Lemma 5 of \cite{bertsekas2000gradient}.
 \end{proof}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Using above result,  there exists a $k> k_0$ such that  $k \in S $ and indicator function $\chi_k =1$. Therefore,
 $$
 \lim_{k \to \infty} \sup \| \nabla J( \bm{\theta}_k)\| \leq \delta.
 $$  Therefore, for $k>k_0$, we get
   \begin{align}
 J (\bm{\bm{\theta}}_{k+1}) \geq &  J (\bm{\bm{\theta}}_{k}) - \chi_{k} \left\{  \alpha_k\bm{w}_k ^\top  \nabla J(\bm{\theta}_k)   + \alpha_k^2 L_1(J) \left\|  \bm{w}_k  \right\|^2\right\}. 
 \end{align}
Now following  Lemma 3 of  \cite{bertsekas2000gradient},  $\chi_{k} \left\{  \alpha_k \bm{w}_k ^\top  \nabla J(\bm{\theta}_k)   + \alpha_k^2 L_1(J) \left\| \bm{w}_k  \right\|^2\right\}$ converges. Further, using Propostion \ref{prop:1} with $W_k=0   \,  \forall k$ and $Z_k=\chi_{k} \left\{  \alpha_k \bm{w}_k ^\top  \nabla J(\bm{\theta}_k)   + \alpha_k^2 L_1(J) \left\|  \bm{w}_k  \right\|^2\right\} ,$  $J(\bm{\theta}_k)$ converges to a finite value $ J(\bm{\theta}^*)$ and $\nabla J(\bm{\theta}^*)=0$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  Evaluating expectation of  \eqref{eqn_Jre}, we get
   \begin{align}
\mathbb{E} \left[  J (\bm{\bm{\theta}}_{k+1}) \right]  \geq & \mathbb{E} \left[  J (\bm{\bm{\theta}}_{k}) \right] + \alpha_k  \mathbb{E} \left[  \| {\nabla} J (\bm{\bm{\theta}}_k) \|^2 \right]  \nonumber \\
&- \alpha_k^2 L_1(J)  \mathbb{E} \left[ \left\| \bm{w}_k  \right\|^2\right]. 
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  Now using the assumption on the noise sequence, $w_k$  in the above expression
  \begin{align}
& \mathbb{E} \left[  J (\bm{\bm{\theta}}_{k+1}) \right]  \geq & \mathbb{E} \left[  J (\bm{\bm{\theta}}_{k}) \right] + \alpha_k (1-L\alpha_k Y_2)  \mathbb{E} \left[  \| {\nabla} J (\bm{\bm{\theta}}_k) \|^2 \right] \nonumber \\ & - \alpha_k^2 L_1(J)  Y_1. 
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 With  $  (1-L\alpha_k Y_2) \approx 1$, 
   \begin{align}
\mathbb{E} \left[  J (\bm{\bm{\theta}}_{k+1}) \right]  \geq & \mathbb{E} \left[  J (\bm{\bm{\theta}}_{k}) \right] + \alpha_k  \mathbb{E} \left[  \| {\nabla} J (\bm{\bm{\theta}}_k) \|^2 \right]  - \alpha_k^2 L_1(J)  Y_1 
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 Rearranging the above expression yields
    \begin{align}
\mathbb{E} \left[  \| {\nabla} J (\bm{\bm{\theta}}_k) \|^2 \right]   \leq & \frac{1}{\alpha_k} \left(  \mathbb{E} \left[  J (\bm{\bm{\theta}}_{k+1}) \right] - \mathbb{E} \left[  J (\bm{\bm{\theta}}_{k}) \right]   \right)    + \alpha_k  L_1(J)  Y_1
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 Let $\bar{k} = k-k_0$, now summation on both sides from 1 to N gives, 
    \begin{align}
& \sum_{\bar{k}=1}^{N}  \mathbb{E} \left[  \| {\nabla} J (\bm{\bm{\theta}}_{\bar{k}}) \|^2 \right]   \leq  \sum_{\bar{k}=1}^{N}  \left( \frac{1}{\alpha_{\bar{k}}} -  \frac{1}{\alpha_{\bar{k}-1}} \right) \mathbb{E}  \left[  J (\bm{\bm{\theta}}_{{\bar{k}}}) \right] \nonumber \\ &+ \frac{1}{\alpha_N} \mathbb{E} \left[  J (\bm{\bm{\theta}}_{{{N+1}}}) \right]       + \frac{1}{\alpha_0} \mathbb{E} \left[  J (\bm{\bm{\theta}}_{{{0}}}) \right]  + \sum_{\bar{k}=1}^{N} \alpha_{\bar{k}} L_1(J)  Y_1
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 Now using Jenson's inequality, we get
     \begin{align}
& \sum_{\bar{k}=1}^{N}  \mathbb{E} \left[  \| {\nabla} J (\bm{\bm{\theta}}_{\bar{k}}) \|^2 \right]   \leq  \sum_{\bar{k}=1}^{N}  \left( \frac{1}{\alpha_{\bar{k}}} -  \frac{1}{\alpha_{\bar{k}-1}} \right) \mathbb{E}  \left[ | J (\bm{\bm{\theta}}_{{\bar{k}}})| \right] \nonumber \\ &+ \frac{1}{\alpha_N} \mathbb{E} \left[ | J (\bm{\bm{\theta}}_{{{N+1}}}) | \right]       + \frac{1}{\alpha_0} \mathbb{E} \left[ | J (\bm{\bm{\theta}}_{{{0}}})| \right]  + \sum_{\bar{k}=1}^{N} \alpha_{\bar{k}} L_1(J)  Y_1
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 Using upper bound of the  cost function in the above expression along with step-size $\alpha_k$ of the form $ k^{-b},  \, b \in (0,1)$, we get
      \begin{align}
\sum_{\bar{k}=1}^{N}  \mathbb{E} \left[  \| {\nabla} J (\bm{\bm{\theta}}_{\bar{k}}) \|^2 \right]   \leq & \frac{2 U_R}{\alpha_{N}(1-\gamma)} +L Y_1 + \frac{LY_1}{1-b} (N^{1-b}-1)
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Dividing the above expression throughout by $N$ and  using $\alpha_N = N^{-b} $ 
       \begin{align} 
& \frac{1}{N} \sum_{\bar{k}=1}^{N}  \mathbb{E} \left[  \| {\nabla} J (\bm{\bm{\theta}}_{\bar{k}}) \|^2 \right]   \leq & \frac{2 U_R}{(1-\gamma)}  N^{b-1} +L Y_1 + \nonumber \\ & \frac{LY_1b}{N(1-b)} (N^{1-b}-1) \label{eqn:35}
 \end{align}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 The above expression implies first-order convergence to a stationary point, in other words, gradient of cost function settles to a constant value  using the proposed approach with variable step-size. Expression \eqref{eqn:35} can be further used to evaluate the order of complexity of the proposed algorithm. \\
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\| \mathbf{g}_{\mu}(\bm{\theta}_k) \|^2 & = \left\|\frac{1}{1-\gamma} {\mathbb{E}_{(s,a) \sim  (1-\gamma) \rho_{\pi_{\bm{\theta}_k}}(s) \pi_{\bm{\theta}_k}  }  \left[ \hat{Q}_{\pi_{\theta}}(s,a)  \mathbb{E}_{\mathbf{u}}\left[ \frac{L_{\pi} (\bm{\bm{\theta}}+\mu \mathbf{u},s)- L_{\pi} (\bm{\bm{\theta}},s) }  {\mu} \right] \right]}\right\|^2 
%\end{align}

==> sections/policysearch.tex <==
%!TEX root = main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Exploratory Policy Search}
Conventional approach to policy characterization uses a Gaussian policy with constant variance and assumes bounded state-action space and  parameter set in order to prevent destructively large policy updates and unbounded score functions.   For scenarios that are likely to unpredictable events with severe consequences (Black swan effect), these standard distributions are inadequate.  For instance,  consider a scenario where a  high positive reward is only obtained when the agent achieves a specific goal and it receives a relatively small positive reward when it reaches an intermediate goal. In such scenarios, the agent needs to explore the extreme action space in order to learn the policy effectively.  Standard policy models are inadequate for such extreme departures. Further, standard policy assumptions of  Reinforced Learning (RL)  algorithms no longer holds. 
\\
In order to model these misaligned myopic and farsighted decision models, we propose to use a  class of heavy-tailed distributions,  $\alpha$ stable distribution [].  Symmetric $\alpha$ stable distributions generalize Gaussian policies with $\alpha$ defining the heaviness of the tail of the distribution. A value of $\alpha=2$ corresponds to Gaussian policy 
\begin{align*}
\pi_{\bm{\theta}}(a|s) = \mathcal{N} (a|s^\top \bm{\theta}, \sigma^2),
\end{align*}
and lower values result in heavy-tailed policies. We present a representative   example for $\alpha$ stable distributions with $\alpha<2$. \\
\textbf{ Example:} Consider an $\alpha$ stable distribution with  $\alpha=1$. Here we get a  Cauchy distribution, a variant of the power-law distribution with a probability distribution 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
\pi_{\bm{\theta}}(a|s) = \frac{1}{\sigma \pi (1+((a-x_0)/\sigma)^2) },
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where, $x_0$ is the mode of the distribution and $\sigma$ is the scale, $\bm{\theta}=[\bm{\theta}_{x_0}, \bm{\theta}_{\sigma}]$, $x_0$ and $\sigma$ are functions of $\bm{\theta}$ and $x_0 $ with $x_0=  \bm{\theta}_{x_0}^\top s$, $\sigma = \exp^{\bold{1}^\top \bm{\theta}_{\sigma}}$.  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%comment
Log-likelihood of probability distribution can be expressed as
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\begin{align}
& L_{\pi_{\bm{\theta}}}(s,a): = \log \pi_{\bm{\theta}}(a|s)  \nonumber \\ & = -\log \left( \exp^{\bold{1}^\top \bm{\theta}_{\sigma}} \pi \left(1+\left(\frac{(a-\bm{\theta}_{x_0}^\top s)}{\exp^{\bold{1}^\top \bm{\theta}_{\sigma}}}\right)^2\right) \right),
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where, $\bm{\theta}=[\bm{\theta}_{x_0}, \bm{\theta}_{\sigma}]^\top \in \mathbb{R}^{d} $.\\\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Heavy tailed variants result in unbounded score function and policy divergence  as discussed above. Moreover, a variable scale ($\sigma $) to prevent  sub-optimal solutions further degrades  stability of policy updates [cite]. \\\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
Therefore,  we propose an adaptive variance for $\alpha$ stable policy updates using a projected variant of policy gradients. Following the proximal approach to  policy gradients, a surrogate objective function takes the form [cite]%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
& L^s(\bm{\theta}) = \mathbb{E} \left[\min\left\{ \frac{\pi_{\bm{\theta}}(a_t|s_t)}{\pi_{\bm{\theta_{\textrm{old}}}}(a_t|s_t)} Q^{\pi_{\theta}}(s_t,a_t), \right. \right. \nonumber 
\\
& \left. \left. \textrm{clip}(\frac{\pi_{\bm{\theta}}(a_t|s_t)}{\pi_{\bm{\theta_{\textrm{old}}}}(a_t|s_t)} (s_t,a_t),1-\epsilon, 1+\epsilon) Q^{\pi_{\theta} } \right\}\right]  
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We propose to implement the  above surrogate objective  using a clipped variant of score function
\begin{align}
& \nabla L^{\textrm{clip}}(\bm{\theta}) = \textrm{clip}  \left(\nabla L(\bm{\theta}) , 1-\epsilon, 1+\epsilon \right) 
\end{align}
The modified score function  removes the incentive when the objective between successive updates moves outside the  bounds  $(1-\epsilon, \, 1+\epsilon)$. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
An unbiased estimate of $Q-$ function can be  obtained using 
Monte-Carlo roll-outs for a time  horizon $T^{'} \sim  \textrm{Geom}(1 -\gamma^{1/2})$  as follows \cite{zhang2019convergence} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
& \hat{Q}_{{\pi}_{\bm{\theta}} } (s,a) = \sum_{t=0}^{T^{'}}  \gamma^{t/2} R(s_t,a_t),  \nonumber\\ &  s_0=s, a_0=a, \, T^{'}: =\textrm{Geom}(1 -\gamma^{1/2})
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The proposed algorithm  for exploratory policy search with adaptive variance  is summarized in Algorithm \ref{Algorithm1}. 


 


  \begin{algorithm}[t]
\begin{algorithmic}
%\textbf{Procedure:}{Require: Step-size $\alpha_k$}
 \STATE \textbf{Initialize} :   Initial policy parameter,  $\bm{\theta}_0, \ k=1$, $\epsilon$, $\gamma$ \\
\textbf{Repeat:}
   \STATE Simulate  trajectories, $\tau_k =(s_0,a_0, s_1,a_1, \ldots)$ by $\pi_{\bm{\theta_k}}(.|s)$
  \STATE Draw $T$  from the geometric distribution Geom($1 -\gamma^{1/2})$, i.e.,  $ P (T = t) = (1 -\gamma^{1/2}) \gamma^{t/2}$, initialize $\hat{Q}=0$
 \FOR  {$t = 0, \ldots, T-1$} 
  \STATE Collect and add the instantaneous reward $R(s_t, a_t)$ to $\hat{Q}$ 
\STATE $\hat{Q}    \leftarrow  \hat{Q} + \gamma^{t/2} R(s_t, a_t)$
\ENDFOR
\FOR {$(s_t,a_t)  \in \tau_k$}
\STATE Obtain  score function,  ${\nabla} L_{\pi_{\bm{\theta}_k}}$
\STATE ${\nabla} L_{\pi_{\bm{\theta}_k}} \leftarrow \min\left\{  {\nabla} L_{\pi_{\bm{\theta}_k}} , \textrm{clip}({\nabla} L_{\pi_{\bm{\theta}_k}} , (1-\epsilon, 1+\epsilon) \right\}$
 \STATE Update policy parameter,  $\bm{\theta}_{k+1} \leftarrow \bm{\theta}_{k} + \alpha_k  \hat{Q}(s_t,a_t) {\nabla} L_{\pi_{\bm{\theta}_k}}   $
\STATE $k \leftarrow k+1$
\ENDFOR
 
 \textbf{ Until Convergence}
  % \EndProcedure
   \STATE \textbf{Return: $\bm{\theta}_k$}\\

 \end{algorithmic}
  \caption{Exploratory Policy Search with adaptive Variance}
 \label{Algorithm1}
 \end{algorithm}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% score function for Cauchy
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%The score function of the policy gradient is given by 
%\begin{align}
%\nabla_{\bm{\theta}} L_{\pi_{\bm{\theta}}}(s,a) = \left[
%\begin{matrix}
% \frac{2}{1+ \left( \frac{(a-\bm{\theta}_{x_0}^\top s)}{\sigma}\right)^2} \left(  \frac{(a-\bm{\theta}_{x_0}^\top s)}{\sigma} \right)  s
% \\
% -\bold{1} + \frac{2}{1+ \left( \frac{(a-\bm{\theta}_{x_0}^\top s)}{\sigma}\right)^2} \left(a-\bm{\theta}_{x_0}^\top s\right)^2 \sigma^{-2} 
%\end{matrix}
%\right].
%\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

